ChatGPT Inaccuracy Mitigation during Technical Report Understanding: Are We There Yet?

Hallucinations, the tendency to produce irrelevant/incorrect responses, are prevalent concerns in generative AI-based tools like ChatGPT. Although hallucinations in ChatGPT are studied for textual responses, it is unknown how ChatGPT hallucinates for technical texts that contain both textual and technical terms. We surveyed 47 software engineers and produced a benchmark of 412 Q&A pairs from the bug reports of two OSS projects. We find that a RAG-based ChatGPT (i.e., ChatGPT tuned with the benchmark issue reports) is 36.4% correct when producing answers to the questions, due to two reasons 1) limitations to understand complex technical contents in code snippets like stack traces, and 2) limitations to integrate contexts denoted in the technical terms and texts. We present CHIME (ChatGPT Inaccuracy Mitigation Engine) whose underlying principle is that if we can preprocess the technical reports better and guide the query validation process in ChatGPT, we can address the observed limitations. CHIME uses context-free grammar (CFG) to parse stack traces in technical reports. CHIME then verifies and fixes ChatGPT responses by applying metamorphic testing and query transformation. In our benchmark, CHIME shows 30.3% more correction over ChatGPT responses. In a user study, we find that the improved responses with CHIME are considered more useful than those generated from ChatGPT without CHIME.

==> Discussion.tex <==
\section{Discussion}\label{sec:discussion}
%The findings and observations from the study of CHIME offer valuable insights into the potential and limitations of advanced AI tools in software engineering. 
In the discussion section, we delve into two key aspects: the influence of threshold settings on correctness analysis and the potential threats that could affect the validity of our findings.
%\gias{in this section, we will discuss whether there is any difference in terms of correctness analysis, if we had used different similarity threshold values, we will experiment with thresholds of 0.75, 0.60, 0.65, 0.80, 0.85, 0.90, and 0.95}
\subsection{Analyzing the Impact of Different Similarity Thresholds}
In this section, we investigate the impact of varying similarity threshold values on correctness analysis. We experiment with different threshold values ranging from 0.60 to 0.95 for summarization questions. Figure \ref{fig:threshold_analysis} presents the results for different components at each threshold.  It is worth noticing that each component demonstrate noticeable fluctuations in correctness rates across different thresholds. Lower thresholds increase the likelihood of capturing relevant information but also raise the risk of including noise or irrelevant data. On the other hand, higher thresholds may improve precision by filtering out irrelevant information but could lead to missed opportunities for relevant insights. After conducting a analysis of accuracy rates across various similarity threshold values of CHIME, we have chosen the threshold of 0.7 as it gives the highest accuracy. This value represents an optimal trade-off between capturing sufficient relevant information and minimizing false positives.

\begin{figure}
    \centering
    \begin{tikzpicture}
    \begin{axis}[
        xlabel={Threshold},
        %ylabel={ (\%)},
        xmin=0.6, xmax=0.95,
        ymin=0, ymax=95,
        xtick={0.6,0.65,0.7,0.75,0.8,0.85,0.9,0.95},
        ytick={10,20,30,40,50,60,70,80,90},
        ytick style={opacity=0},
        yticklabel={\pgfmathprintnumber{\tick}\%},
        %legend pos=north east,
        %legend style={
        %at={(1,1.27)},
        %anchor=north east,
        %legend columns=3,
        %font=\small,
        %draw=none,
        %/tikz/every even column/.append style={column sep=0.2cm}
    %},
        %legend style={at={(1.1,0.5)},anchor=east},
        %ymajorgrids=true,
        legend style={
        at={(0.5,1.2)},
        anchor=north,
        legend columns=4,
        font=\footnotesize,
        draw=none,
        row sep=0.2em,
        column sep=0.5em,
        /tikz/every even column/.append style={column sep=0.5em}, % Adjust spacing for even columns
        %width=0.5\linewidth, % Specify the width of the legend
    },
        grid style=dashed,
    ]
    
    % LLM line
    \addplot[color=red] coordinates {
        (0.6, 52.4)
        (0.65, 47.6)
        (0.7, 38.1)
        (0.75, 35.7)
        (0.8, 21.4)
        (0.85, 19.0)
        (0.9, 0.0)
        (0.95, 0.0)
    };
    \addlegendentry{GPT}
    
    % CFG line
    \addplot[color=cyan, mark=*] coordinates {
        (0.6, 52.4)
        (0.65, 45.2)
        (0.7, 35.7)
        (0.75, 28.6)
        (0.8, 21.4)
        (0.85, 11.9)
        (0.9, 0.0)
        (0.95, 0.0)
    };
    \addlegendentry{CFG}
    
    % Query line
    \addplot[color=orange, mark=*] coordinates {
        (0.6, 57.1)
        (0.65, 47.6)
        (0.7, 35.7)
        (0.75, 21.4)
        (0.8, 14.3)
        (0.85, 9.5)
        (0.9, 2.4)
        (0.95, 0.0)
    };
    \addlegendentry{Query}
 \begin{comment}
     
    % MT line
    \addplot[color=orange, mark=*] coordinates {
        (0.6, 57.1)
        (0.65, 47.6)
        (0.7, 38.1)
        (0.75, 26.2)
        (0.8, 14.3)
        (0.85, 14.3)
        (0.9, 4.8)
        (0.95, 0.0)
    };
    \addlegendentry{MT}
    
    % COVE line
    \addplot[color=purple, mark=*] coordinates {
        (0.6, 40.5)
        (0.65, 31.0)
        (0.7, 26.2)
        (0.75, 23.8)
        (0.8, 19.0)
        (0.85, 14.3)
        (0.9, 0.0)
        (0.95, 0.0)
    };
    \addlegendentry{COVE}
     \end{comment}   
    % COVE_MT line
    \addplot[color=blue, mark=*] coordinates {
        (0.6, 59.5)
        (0.65, 47.6)
        (0.7, 38.1)
        (0.75, 33.3)
        (0.8, 28.6)
        (0.85, 23.8)
        (0.9, 4.8)
        (0.95, 2.4)
    };
    \addlegendentry{RV}
    
    % CHIME line
    \addplot[color=green!30!black, mark=*] coordinates {
        (0.6, 66.7)
        (0.65, 64.3)
        (0.7, 59.5)
        (0.75, 35.7)
        (0.8, 23.8)
        (0.85, 16.7)
        (0.9, 2.4)
        (0.95, 2.4)
    };
    \addlegendentry{CHIME}

    \addlegendimage{color=black,solid}
    \addlegendentry{Correctness}
    \addlegendimage{color=black, dashed}
    \addlegendentry{Accuracy}
    
   \addplot[color=green!30!black, dashdotted, mark=*]
        coordinates {
        (0.6, 80.95)
        (0.65, 85.71)
        (0.7, 90.48)
        (0.75, 69.05)
        (0.8, 61.90)
        (0.85, 54.76)
        (0.9, 40.48)
        (0.95, 40.48)
        };
    \end{axis}
    \end{tikzpicture}
    \caption{Impact of Threshold on Similarity Analysis}
    \label{fig:threshold_analysis}
\end{figure}



\begin{comment}
\subsection{Implications}
\gias{we will shorten the following and move the summary to conclusions. we don't need an implication section here}
The successful implementation and effectiveness of CHIME have several significant implications:

\textbf{Enhanced Accuracy in Technical Contexts}. CHIME demonstrates that with specialized enhancements, AI models like ChatGPT can achieve higher accuracy in technical domains such as software engineering. This suggests a path forward for developing AI tools tailored to specific professional fields.

\textbf{Utility in Real-World Software Development}. The positive response from developers in the study indicates that tools like CHIME can be practically useful in real-world software development, particularly in bug report analysis and resolution. This signifies a step towards more AI-integrated software development processes.

\textbf{Methodological Advancements in AI}. The components of CHIME, such as CFGs, CoVE, and MRs, showcase innovative methods to enhance the reliability and consistency of AI responses. These methodological advancements could be applied to other AI applications beyond software engineering.

\textbf{Improving Human-AI Collaboration}. The study highlights the potential of AI tools to collaborate effectively with human professionals, augmenting their capabilities and improving efficiency. This could reshape the dynamics of team-based work in various industries.

Setting Standards for AI Tools in Technical Domains: CHIME’s approach to addressing specific challenges in software engineering sets a precedent for how AI tools can be designed and evaluated for other technical domains.

\end{comment}
\subsection{Threats to Validity}
In assessing the validity of our study on CHIME, several potential threats must be considered. Firstly, the selection of issues from the OpenJ9 and ElasticSearch repository may introduce a selection bias, affecting the generalizability of the findings across various software engineering contexts. The participant pool, consisting of developers, might not comprehensively represent the diverse perspectives and experiences found in the broader software engineering community, leading to a potential participant bias. The benchmark's design, while extensive, may not encompass all possible software issue types or scenarios, potentially limiting the study's scope and applicability. Furthermore, CHIME's reliance on ChatGPT’s underlying model means that any inherent limitations or biases in ChatGPT could influence CHIME’s performance. The dynamic and evolving nature of software development also poses a challenge, as current issues or technologies may change over time, impacting the long-term relevance of our findings. Finally, the methodology used for evaluating CHIME could affect the accuracy and objectivity of our effectiveness assessment. Acknowledging and addressing these threats is vital for a balanced interpretation of the study results and for guiding future advancements in AI tools within software engineering and related fields.








==> marcos.tex <==
\usepackage{fancybox}
\usepackage{tcolorbox}

\makeatletter


\newcommand{\review}[1]{{\textit{#1}}~\\}
\newcommand{\respto}[1]{
\fcolorbox{black}{black!15}{
\label{response:#1}
\bf
  \scriptsize Review {#1}}~
}
\newcommand{\citerespexp}[1]{
\fcolorbox{black}{black!15}{
 \bf
  \scriptsize Review {#1}}~{\bf{on page \pageref{response:#1}}}
}

\newcommand{\citerespexpnopage}[1]{
\fcolorbox{black}{black!15}{
 \bf
  \scriptsize Review {#1}}
}

\newcommand{\citeresp}[1]{
\fcolorbox{black}{black!15}{
 \bf
  \scriptsize Review {#1}}
}


\newcommand{\mybox}[1]{%
	\setbox0=\hbox{#1}%
	\setlength{\@tempdima}{\dimexpr\wd0+13pt}%
	\begin{tcolorbox}[boxrule=0.5pt, colback=gray!10, arc=4pt,
		left=6pt,right=6pt,top=6pt,bottom=6pt,boxsep=0pt]
		#1
	\end{tcolorbox}
}

\newcommand{\myboxwithheaders}[2]{
    \begin{tcolorbox}[
        colback=white,
        colframe=black,
        coltitle=black,
        title={\textbf{#1}},
        title filled,
        colbacktitle=lightgray,
        boxrule=0.5pt
    ]
        #2
    \end{tcolorbox}
}

\newcommand{\myboxwithheader}[2]{
    \begin{tcolorbox}[
        colback=white,
        colframe=black,
        coltitle=black,
        title={\textbf{#1}},
        title filled,
        colbacktitle=lightgray,
        boxrule=0.5pt,
        %segmentation style={solid, draw=none}, % Remove the draw option
    ]
        %\colorbox{red!20}{\parbox{\dimexpr\linewidth+3\fboxsep}{#2}}

    \end{tcolorbox}
}
\newcommand{\custombarchartwithvalue}[4]{%
    \begin{tikzpicture}[xscale=#4,yscale=.2]
    % Calculate total
    \pgfmathsetmacro{\Total}{int(#1+#2+#3)}

    % Draw the bars
    \fill[gray!20] (0,0) rectangle (#1,1);
    \fill[gray!40] (#1,0) rectangle (#1+#2,1);
    \fill[gray!60] (#1+#2,0) rectangle (\Total,1);

    % Add text inside the bars
        \ifnum#1>0
        \node at (#1/2,0.5) {{#1}};
    \fi
    %\node at (#1/2,0.5) {#1};
    \node at (#1+#2/2,0.5) {{#2}};
    \node at (#1+#2+#3/2,0.5) {{#3}};
    % Add total at the end
    \node[right] at (\Total,0.5) {\textbf{\Total}};
    \end{tikzpicture}
}

\definecolor{SoftGreen}{HTML}{9BC2B2}
\definecolor{WarmBrown}{HTML}{D4B996}
\definecolor{LightBlue}{HTML}{AED9E0}
\definecolor{PaleYellow}{HTML}{F3EACB}
\definecolor{GentleGray}{HTML}{D9D9D9}

\newcommand{\custombarchartwithvaluetwobar}[2]{%
    \begin{tikzpicture}[xscale=0.05,yscale=.3]
    % Calculate total
    \pgfmathsetmacro{\Total}{int(#1+#2)}

    % Draw the bars
    \fill[gray!30] (0,0) rectangle (#1,1);
    \fill[gray!60] (#1,0) rectangle (#1+#2,1);
    %\fill[teal!30] (#1+#2,0) rectangle (\Total,1);

    % Add text inside the bars
        \ifnum#1>0
        \node at (#1/2,0.5) {{#1\%}};
    \fi
    %\node at (#1/2,0.5) {#1};
    \node at (#1+#2/2,0.5) {{#2\%}};
    %\node at (#1+#2+#3/2,0.5) {{#3}};
    % Add total at the end
    %\node[right] at (\Total,0.5) {\textbf{\Total}};
    \end{tikzpicture}
}



\tcbset{qa_box/.style={
    colback=white,
    colframe=black,
    coltitle=black,
    title filled,
    colbacktitle=lightgray,
    boxrule=0.5pt,
    left=10pt,
    right=10pt,
    boxsep=0pt,
    late options/.try,
}}

\tcbset{qa_box-rootbox/.style={
    qa_box,
    colback=gray!40,
}}
\tcbset{qa_box-question/.style={
    sharp corners,
    qa_box,
    oversize,
    colback=white!10,
    top=10pt,
}}
\tcbset{qa_box-response/.style={
    sharp corners=north,
    oversize,
    qa_box,
    colback=lightgray!30,
}}


\tcbset{every box on layer 2/.append style={
  late options/.style={
    left=10pt,
    right=10pt,
  }
}}


\newcommand{\qabox}[3]{
    \begin{tcolorbox}[qa_box-rootbox, size=small]
        \textbf{#1}
        \begin{tcolorbox}[qa_box-question, size=small]
            #2
        \end{tcolorbox}
        \vspace{-13pt}
        \begin{tcolorbox}[qa_box-response, size=small]
            #3
        \end{tcolorbox}
        \vspace{-13pt}
    \end{tcolorbox}
}

% --- for revision
\newcommand{\rev}[1]{\textcolor{purple}{\st{#1}}}
%\newcommand{\rev}[1]{}   
\newcommand{\add}[1]
{
\textcolor{blue}{\textbf{
#1
}}}
%\newcommand{\add}[1]{{#1}}

% todo commands:
\newcommand{\todoc}[2]{{\textcolor{#1}{\textbf{#2}}}}
\newcommand{\todored}[1]{\todoc{red}{\textbf{[[#1]]}}}
\newcommand{\todogreen}[1]{\todoc{green}{\textbf{[[#1]]}}}
\newcommand{\todoblue}[1]{\todoc{blue}{\textbf{[[#1]]}}}
\newcommand{\todogray}[1]{\todoc{Gray}{\textbf{[[#1]]}}}
\newcommand{\todoorange}[1]{\todoc{orange}{\textbf{[[#1]]}}}
\newcommand{\todobrown}[1]{\todoc{brown}{\textbf{[[#1]]}}}
\newcommand{\todopurple}[1]{\todoc{purple}{\textbf{[[#1]]}}}

\newcommand{\todo}[1]{\todored{TODO: #1}}
\newcommand{\song}[1]{\todoorange{Song: #1}}
\newcommand{\tool}{\textit{CIMBUR}}



\newcommand{\customTwoBarChartwithlimit}[8]{%
\pgfmathsetmacro{\resultxmin}{#2 + #3}
\pgfmathsetmacro{\resultxminnext}{#5 + #6}
\begin{figure}[h]
%%%%%%%%%%%%%%%%% plot on both side 
    \centering
    \hspace{-2cm}
    %\hspace{-1.8cm}
    %\begin{subfigure}[b]{.2\columnwidth}
    \begin{subfigure}[b]{.3\columnwidth}
        \centering
    \begin{tikzpicture}[scale=0.6]
        \begin{axis}[
            xbar stacked,   % Stacked horizontal bars
            xmin=\resultxmin,         % Start x-axis at 0 for positive values
            xmax=#1,        % End x-axis at 88 for positive values
            hide y axis,      % Hide the y-axis
            axis x line*=bottom, % Middle x-axis
            %axis lines*=middle, % Draw the axis in the middle of the chart
            %axis on top,    % Draw axis lines on top of bars
            %ytick=data,     % Tick marks at data points
            %ytick style={font=\large},
            width=8cm,        % Width of the plot
            height=20mm,      % Height of the plot
            %ytick=\empty,
            %yticklabels={},%${Analysis-S (T1)},    
            y dir=reverse,  % Reverse the y-axis to start with the first label on top
            legend style={at={(0.5,2.65)},anchor=north,legend columns=-1,draw=none}, % Legend below the plot
            %xtick={38,20,0,20,40,60,80}, % Define specific ticks
            xticklabels={20\%,0,20\%,40\%,60\%}, % Label them as from 38 to 88
            xticklabel style={anchor=north}, % Style the tick labels appropriately
            %enlarge y limits={abs=0.35},
            %enlarge x limits=0.01, % Add space between bars
            tick align=center,
            %ytick pos=left,
            %xlabel=Percentage (\%),
            bar width = 15pt,
            extra x ticks={0}, % Define extra ticks
            extra x tick style={ % Style the extra ticks
                grid=major,
                grid style={black},
                tick label style={anchor=north},
                %tick style={line width=2pt}
            },
        ]
        % Neutral values (center)
        \addplot+[xbar, fill=lightgray!90!white, draw=lightgray!90!white, mark=none,forget plot] coordinates {(#2,0)};        
        % Negative valuustomTwoBarChartes (left side)
        \addplot+[xbar, fill=orange!85!white, draw=orange!85!white, mark=none, forget plot] coordinates {(#3,0)};
        % Positive values (Right side)
        \addplot+[xbar, fill=cyan!95!white, draw=cyan!95!white, mark=none, forget plot] coordinates {
            (#1,0)
        };

        
        \addlegendimage{orange,fill=orange}
        \addlegendentry{No}
        \addlegendimage{lightgray,fill=lightgray}
        \addlegendentry{Maybe}
        \addlegendimage{cyan,fill=cyan}
        \addlegendentry{Yes}
        \end{axis}
    \end{tikzpicture} 
    %\caption{}
    \label{fig:task-interest}
    \end{subfigure}
%\hspace{3.9cm}
\hspace{1.5cm}
    \begin{subfigure}[b]{.2\columnwidth}
    %\begin{subfigure}[b]{.2\columnwidth}
        \centering
        \begin{tikzpicture}[scale=0.6]
            \begin{axis}[
                xbar stacked,   % Stacked horizontal bars
                xmin=\resultxminnext,         % Start x-axis at 0 for positive values
                xmax=#4,        % End x-axis at 88 for positive values
                %axis lines*=middle, % Draw the axis in the middle of the chart
                %axis on top,    % Draw axis lines on top of bars
                hide y axis,      % Hide the y-axis
                axis x line*=bottom, % Middle x-axis
                width=8cm, 
                height=20mm,
                %ytick=\empty,     % Tick marks at data points
                %yticklabels={},
                %ylabel={},
                y dir=reverse,  % Reverse the y-axis to start with the first label on top
                legend style={at={(0.5,2.65)},anchor=north,legend columns=-1,draw=none}, % Legend below the plot
                %xtick={38,20,0,20,40,60,80}, % Define specific ticks
                xticklabels={20\%,0,20\%,40\%,60\%,80\%}, % Label them as from 38 to 88
                xticklabel style={anchor=north}, % Style the tick labels appropriately
               %enlarge y limits={abs=0.35},
                %enlarge x limits=0.01, % Add space between bars
                tick align=center,
                ytick pos=left,
                %xlabel=Percentage (\%),
                bar width = 15pt,
                extra x ticks={0}, % Define extra ticks
                extra x tick style={ % Style the extra ticks
                    grid=major,
                    grid style={black},
                    tick label style={anchor=north},
                    %tick style={line width=2pt}
                },
            ]

            \addplot+[xbar, fill=yellow!90!black, draw=yellow!90!black, mark=none, forget plot] coordinates {
                (#5,0)
                
            };
            
            % "No" values (Orange), added after "Yes" values to stack correctly
            \addplot+[xbar, fill=red!90, draw=red!90, mark=none, forget plot] coordinates {
               (#6,0)
            };

            % "Yes" values (Cyan)
            \addplot+[xbar, fill=green!70!black, draw=green!70!black, mark=none, forget plot] coordinates {
                (#4,0)
            };

            % "Maybe" values (Light Gray), added last


            \addlegendimage{red,fill=red}
            \addlegendentry{Not Useful}
            \addlegendimage{yellow,fill=yellow}
            \addlegendentry{Neutral}
            \addlegendimage{green,fill=green}
            \addlegendentry{Useful}
            \end{axis}
        \end{tikzpicture}
        %\caption{}
        \label{fig:task-usefulness}
    \end{subfigure}
    \vspace{-0.5cm}
   \caption{(a) Interest for #7 (b) Usefulness Perception of #7}
   \label{#8}
   \vspace{-0.1cm}
\end{figure}
}


\newcommand{\customTwoBarChartwithlimitanother}[8]{%
\pgfmathsetmacro{\resultxmin}{#2 + #3}
\pgfmathsetmacro{\resultxminnext}{#5 + #6}
\begin{figure}[!h]
%%%%%%%%%%%%%%%%% plot on both side 
    \centering
    \hspace{-2cm}
    %\hspace{-1.8cm}
    %\begin{subfigure}[b]{.2\columnwidth}
    \begin{subfigure}[b]{.3\columnwidth}
        \centering
    \begin{tikzpicture}[scale=0.6]
        \begin{axis}[
            xbar stacked,   % Stacked horizontal bars
            xmin=\resultxmin,         % Start x-axis at 0 for positive values
            xmax=#1,        % End x-axis at 88 for positive values
            hide y axis,      % Hide the y-axis
            axis x line*=bottom, % Middle x-axis
            %axis lines*=middle, % Draw the axis in the middle of the chart
            %axis on top,    % Draw axis lines on top of bars
            %ytick=data,     % Tick marks at data points
            %ytick style={font=\large},
            width=8cm,        % Width of the plot
            height=20mm,      % Height of the plot
            %ytick=\empty,
            %yticklabels={},%${Analysis-S (T1)},    
            y dir=reverse,  % Reverse the y-axis to start with the first label on top
            legend style={at={(0.5,2.65)},anchor=north,legend columns=-1,draw=none}, % Legend below the plot
            %xtick={38,20,0,20,40,60,80}, % Define specific ticks
            xticklabels={20\%,0,20\%,40\%,60\%}, % Label them as from 38 to 88
            xticklabel style={anchor=north}, % Style the tick labels appropriately
            %enlarge y limits={abs=0.35},
            %enlarge x limits=0.01, % Add space between bars
            tick align=center,
            %ytick pos=left,
            %xlabel=Percentage (\%),
            bar width = 15pt,
            extra x ticks={0}, % Define extra ticks
            extra x tick style={ % Style the extra ticks
                grid=major,
                grid style={black},
                tick label style={anchor=north},
                %tick style={line width=2pt}
            },
        ]
        % Neutral values (center)
        \addplot+[xbar, fill=lightgray!90!white, draw=lightgray!90!white, mark=none,forget plot] coordinates {(#2,0)};        
        % Negative values (left side)
        \addplot+[xbar, fill=orange!85!white, draw=orange!85!white, mark=none, forget plot] coordinates {(#3,0)};
        % Positive values (Right side)
        \addplot+[xbar, fill=cyan!95!white, draw=cyan!95!white, mark=none, forget plot] coordinates {
            (#1,0)
        };

        
        \addlegendimage{orange,fill=orange}
        \addlegendentry{No}
        \addlegendimage{lightgray,fill=lightgray}
        \addlegendentry{Maybe}
        \addlegendimage{cyan,fill=cyan}
        \addlegendentry{Yes}
        \end{axis}
    \end{tikzpicture} 
    %\caption{}
    \label{fig:task-interest}
    \end{subfigure}
%\hspace{3.9cm}
\hspace{1.5cm}
    \begin{subfigure}[b]{.2\columnwidth}
    %\begin{subfigure}[b]{.2\columnwidth}
        \centering
        \begin{tikzpicture}[scale=0.6]
            \begin{axis}[
                xbar stacked,   % Stacked horizontal bars
                xmin=\resultxminnext,         % Start x-axis at 0 for positive values
                xmax=#4,        % End x-axis at 88 for positive values
                %axis lines*=middle, % Draw the axis in the middle of the chart
                %axis on top,    % Draw axis lines on top of bars
                hide y axis,      % Hide the y-axis
                axis x line*=bottom, % Middle x-axis
                width=8cm, 
                height=20mm,
                %ytick=\empty,     % Tick marks at data points
                %yticklabels={},
                %ylabel={},
                y dir=reverse,  % Reverse the y-axis to start with the first label on top
                legend style={at={(0.5,2.65)},anchor=north,legend columns=-1,draw=none}, % Legend below the plot
                %xtick={38,20,0,20,40,60,80}, % Define specific ticks
                xticklabels={40\%,20\%,0,20\%,40\%,60\%,80\%}, % Label them as from 38 to 88
                xticklabel style={anchor=north}, % Style the tick labels appropriately
               %enlarge y limits={abs=0.35},
                %enlarge x limits=0.01, % Add space between bars
                tick align=center,
                ytick pos=left,
                %xlabel=Percentage (\%),
                bar width = 15pt,
                extra x ticks={0}, % Define extra ticks
                extra x tick style={ % Style the extra ticks
                    grid=major,
                    grid style={black},
                    tick label style={anchor=north},
                    %tick style={line width=2pt}
                },
            ]

            \addplot+[xbar, fill=yellow!90!black, draw=yellow!90!black, mark=none, forget plot] coordinates {
                (#5,0)
                
            };
            
            % "No" values (Orange), added after "Yes" values to stack correctly
            \addplot+[xbar, fill=red!90, draw=red!90, mark=none, forget plot] coordinates {
               (#6,0)
            };

            % "Yes" values (Cyan)
            \addplot+[xbar, fill=green!70!black, draw=green!70!black, mark=none, forget plot] coordinates {
                (#4,0)
            };

            % "Maybe" values (Light Gray), added last


            \addlegendimage{red,fill=red}
            \addlegendentry{Not Useful}
            \addlegendimage{yellow,fill=yellow}
            \addlegendentry{Neutral}
            \addlegendimage{green,fill=green}
            \addlegendentry{Useful}
            \end{axis}
        \end{tikzpicture}
        %\caption{}
        \label{fig:task-usefulness}
    \end{subfigure}
    \vspace{-0.5cm}
   \caption{(a) Interest for #7 (b) Usefulness Perception of #7}
   \label{#8}
   \vspace{-0.1cm}
\end{figure}
}



==> old.tex <==
\section{AI Assistant Needs for Bug Report Exploration}
We surveyed 47 software engineering professionals to explore their preferences and needs for utilizing generative AI chatbots for bug report exploration. This study addresses the following research question (RQs):

%\textbf{RQ1.} Would software practitioners perceive the need for chatbot support during bug report exploration?

\textbf{RQ1.} What types of questions would software practitioners like to ask a chatbot during bug report exploration?

%Additionally, insights from the study guided the development of a comprehensive benchmark aligned with professionals' requirements to evaluate chatbot support during bug report exploration.

%\subsection{Survey Setup to Catalog Questions}
\subsection{Survey Setup}
We present details of the survey setup in this section, including participant demographics and the survey questions.

\subsubsection{Survey Participants} 
We employed the snowball sampling approach to recruit participants from professional network, resulting in 47 professionals taking part, including developers, managers, QA engineers, and others. Notably, the majority of respondents (83\%) held developer roles, indicating a developer-centric perspective in the responses. Regarding experience, the largest proportion of participants (55\%) reported having 4-5 years of experience in the field. Table \ref{tab:demographics} illustrates the distribution of participants across their roles in software industry and years of experience.

\begin{table}
\centering
\caption{Demography of Survey Participants}
\label{tab:demographics}
\renewcommand{\arraystretch}{1.3} % Increase row height

\begin{tabular}{l|ccccc |c}
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{Years of Experience}} \\ \cline{2-7}
\multicolumn{1}{l|}{\textbf{Current Role}} & \textbf{0-3} & \textbf{4-5} & \textbf{6-10} & \textbf{11-15} & \textbf{16-20} & \textbf{Total} \\ \hline
\rowcolor{gray!25}
Developer                                  & 13          & 20           & 4             & 2              & -              & \textbf{39}    \\ %\cline{1-7}
QA Engineer                                & 1           & 1            & -             & -              & -              & \textbf{2}      \\ %\cline{1-7}
\rowcolor{gray!25}
Project Manager                            & -           & 1            & -             & -              & -              & \textbf{1}       \\ %\cline{1-7}
Other                                      & 2           & -            & 2             & -              & 1              & \textbf{5}       \\ \cline{1-7}
\textbf{Total}                             & \textbf{16} & \textbf{22}  & \textbf{6}    & \textbf{2}     & \textbf{1}     & \textbf{47}          
\end{tabular}
\end{table}

Our survey further explored professionals' engagement with Issue Tracking Systems (ITS). It was found that all respondents actively use ITS, such as Jira, GitHub, or in-house systems for several key purposes. The primary reason, cited by 89.36\% of respondents, is issue resolution—addressing and solving bugs; followed by issue triaging, as mentioned by 21 participants, which involves prioritizing and assigning issues.. Project Management - overseeing project progress and coordinating tasks, Reporting - documenting issues for records or stakeholder communication; were also noted as significant reasons for ITS usage. Figure \ref{fig:reason} illustrates the survey responses for the primary reason for issue report interaction.  Also, a vast majority of respondents interact with issue reports on a daily basis (70.21\%). Figure \ref{fig:freq} presents the distribution of issue report interaction frequency. 


\begin{figure}[ht]
    \centering
    \begin{subfigure}{.5\linewidth}
        \centering
        \begin{tikzpicture}
        [pie chart,
        slice type={Daily}{green!30},
        slice type={Weekly}{lime!30},
        slice type={Monthly}{orange!25},
        slice type={Rarely}{red!45},
        pie values/.style={font={\footnotesize}},
        scale=1.1]
        
        \pye{}{70.21/Daily,17.02/Weekly,2.13/Monthly,10.64/Rarely}
        \legend[shift={(-1cm,-1cm)}]{{Daily}/Daily} 
        \legend[shift={(0.5cm,-1cm)}]{{Weekly}/Weekly}
        \legend[shift={(-1cm,-1.3cm)}]{{Monthly}/Monthly}
        \legend[shift={(0.5cm,-1.3cm)}]{{Rarely}/Rarely}
        \end{tikzpicture}
        %\caption{Frequency of Interacting with Issue Reports }
        \caption{}
        \label{fig:freq}
    \end{subfigure}%
    \begin{subfigure}{.5\linewidth}
        \centering
        \begin{tikzpicture}[scale=0.6]
        
            \begin{axis}[
                %title={Primary Reasons for Interaction with Reports},
                ybar,
                xtick distance=1.5,
                %enlargelimits=0.5,
                symbolic x coords={Resolution, Triaging, Reporting, Management },
                xtick=data,
                xticklabel style={font=\large},
                nodes near coords={\pgfmathprintnumber\pgfplotspointmeta\%},
                nodes near coords align={vertical},
                nodes near coords style={font=\large},
                bar width=30pt,
                axis x line*=bottom,
                xtick distance=7,
                y axis line style={opacity=0}, % hide y-axis line
                tickwidth=0pt, % hide ticks
                ytick=\empty,
                width=9cm
                ]
            \addplot[fill=black!30] coordinates {(Resolution,89.36) (Triaging,44.68) (Reporting,36.17) (Management,27.66) };
            
            \end{axis}
        \end{tikzpicture}
        \caption{}
        \label{fig:reason}
    \end{subfigure}
    \caption{(a) Frequency and (b) Primary Reasons of Issue Report Interaction}
    \label{fig:test}
\end{figure}

\subsubsection{Survey Questions}
In this survey, we invited participants to explore and evaluate the prospective utility of an AI chatbot tailored for bug report exploration. Prior to conducting the survey, we sought insights from two seasoned software professionals from a reputable software company, each boasting 16 and 35 years of industry experience. This consultation played a pivotal role in identifying the potential roles and capabilities that an AI chatbot could fulfill within the software development environment. Following extensive discussions on possible topics and question structures, we settled on five distinct topics, spanning from technical diagnostics to operational management, where AI integration could offer assistance. Subsequently, we formulated questions to effectively address each identified topic. These topics include \begin{inparaenum}[T1.]
    \item {\textit{Issue Analytics}}
    \item {\textit{Issue Trends}},
    \item {\textit{Issue Summaries}}
    \item {\textit{Issue Labeling}} and
    \item {\textit{Issue Backlog}}.
\end{inparaenum} 

Initially, participants were prompted to envision an AI chatbot with comprehensive access to bug reports and outline the tasks they envisioned it supporting. Subsequently, they were asked whether they would like to utilize the chatbot for the specified topics (T\#) and to rate the perceived usefulness of each topic for their work. Participants were also asked to rate the potential usefulness of benchmark questions devised for these topics. Lastly, participants were given the opportunity to propose additional topics or questions for integration into the chatbot's benchmark questions and to offer any comments or suggestions for enhancing the existing question set. Given the similarity in question structure across all topics, we condensed the key survey questions into Table \ref{tab:survey_questions} for clarity and ease of reference.

\begin{table}[t!]
\caption{Key Questions (KQ) of the Survey. Here, C/O=Close/Open-ended question, G/S=Generic/Scenario-based question.}
\label{tab:survey_questions}
\centering
\begin{tabular}{c p{5.5cm} c c}
\toprule
\textbf{KQ\#} & \textbf{Questions} & \textbf{O/C} & \textbf{G/S}\\
\midrule
1 & How would you like to utilize a chatbot during bug report exploration?      & O & G\\

2 & Would you want to use the chatbot for T\#?                                  & C & G\\

3 & Rate the usefulness of T\# for your work                                    & C & G\\

4 & Rate the potential usefulness of the following benchmark questions of T\#   & C & S \\

5 & What improvements or new topics could expand the chatbot's benchmark questions? & O & G \\
\bottomrule
\end{tabular}
\end{table}

\begin{comment}
    

\subsection{Desired Functionalities of an AI Chatbot for Bug Report Exploration (RQ1)}
\circled{Q1}
We asked participants to provide a list of tasks and challenges they wish an AI chatbot to address to aid software development and issue management. In exploring the desired functionalities of an AI chatbot for bug report exploration, participants articulated a broad spectrum of advanced features they seek, ranging from basic management aids to sophisticated analytical tools. Through an open coding analysis of participant responses, we can streamline the discussed functionalities into two main categories: Issue Analytics and Issue Management. 

\circled{F1}  \textbf{Issue Analytics} \gias{What is the percentage of responses had this?}focuses on the identification, analysis, and summarization of issues to improve the efficiency of workflows and problem-solving capabilities. This includes tools for identifying duplicate or similar issues to prevent redundant work, support for recognizing and analyzing trends to pinpoint recurring problems, and capabilities for generating concise summaries of issues, aiding developers in understanding and prioritizing their tasks effectively. \gias{with open coding, under issue analytics, you can have sub-topics, each potentially denoting to one or more tasks under RQ2. we need quotes to substantiate each quote}

\gias{follow advice similar to issue analytics above for issue management. why don't we have any tasks mapped to issue management? are you saying that participants were expecting a chatbot to automate their tasks? }
\circled{F2} \textbf{Issue Management} encompasses a range of functionalities aimed at optimizing the management and resolution of issues. This involves effective task management and prioritization features, such as reminders, prioritization of tasks based on severity and requirements, and sprint management. It also includes advanced integration and automation capabilities, like predicting problematic code areas, integrating crash reports into issue trackers, and providing comprehensive summaries and prioritization. Additionally, AI-driven triaging mechanisms for assigning bug reports to suitable developers or teams are crucial for efficient issue distribution and resolution. Beyond these, Issue Management also covers a spectrum of other functionalities, including diagnostic tools, commands for issue reproduction, and suggestions for documentation updates based on recent bug reports, all designed to enhance the efficiency and effectiveness of bug tracking and issue resolution processes. 


\circled{F1} \textbf{Related/Similar Issues: } \color{black!90}\rule{15pt}{6pt} 17.02\%

In response to participant inquiries, there was a collective interest in enhancing the efficiency of issue resolution workflows, particularly regarding the identification and management of similar or duplicate issues and the analysis of recurring problem trends. Participants emphasized the need for tools that could streamline the process of identifying duplicate issues and grouping similar ones together. Features such as flagging potential duplicates or similar issues based on various criteria, were requested to facilitate more effective problem-solving and prevent redundant work. 

\circled{F2} \textbf{Trend Identification:} \color{black!90}\rule{15pt}{6pt} 8.51\%

Participants are willing to get support for highlighting recurring issues, identifying patterns among issues, and analyzing trends to identify recurring problems.

\circled{F3} \textbf{Issue Summarization and Analysis:} \color{black!90}\rule{6pt}{6pt} 10.64\%

Participants highlighted the importance of tools capable of generating concise summaries of multiple issues to aid developers in understanding and prioritizing tasks. Desired functionalities included summarizing issues related to specific queries, providing overviews of issues related to upcoming releases, and summarizing the criticality of open issues. Such features are essential for streamlining communication and decision-making processes within development teams.

\circled{F4} \textbf{Task Management and Prioritization:} \color{black!90}\rule{12pt}{6pt} 19.15%

Participants highlighted the critical importance of effective task management and prioritization features in AI chatbots for optimizing development workflows. Key functionalities identified include reminders for issue resolution, prioritization based on severity and product requirements,  tracking the status and priority of issues and integration of user feedback data to prioritize issues with the greatest impact on users. Additionally, participants emphasized the need for features such as sprint management, which suggests tasks based on time and issue estimations. Furthermore, querying issues with little recent activity and unclear resolution was also deemed essential. 

\circled{F5} \textbf{Integration and Automation:} \color{black!90}\rule{7pt}{6pt} 12.77%


Participants expressed a significant interest in AI chatbots equipped with advanced automation and integration capabilities to streamline issue management processes. They emphasized the importance of features such as automatically predicting problematic code areas, integrating crash reports from Firebase into issue trackers, and providing comprehensive summaries, prioritization, and removal of duplicate reports. Additionally, participants sought functionalities to estimate completion times based on assigned developers, integrate seamlessly with various development tools, and deliver timely notifications and alerts for critical issues. Integration with development tools, such as linking Jira tickets to GitHub pull requests for historical tracking, was also highlighted as essential for improving traceability and collaboration. These functionalities are crucial for enhancing efficiency and productivity in issue resolution workflows, ultimately leading to faster turnaround times and improved software quality.

\circled{F6} \textbf{Triaging:} \color{black!90}\rule{8pt}{6pt} 14.89\%
  
Participants emphasized the need for AI-driven triaging mechanisms to efficiently assign bug reports to suitable developers or teams.  This feature is crucial for streamlining the distribution and resolution of bug reports, ensuring efficient problem-solving and turnaround times.
    
\circled{F7} \textbf{Others:} \color{black!90}\rule{13pt}{6pt} 21.28\%
  
Participants expressed diverse interests in additional functionalities offered by AI chatbots beyond traditional bug tracking. Desired features included providing tips for understanding issue descriptions, handling custom queries, offering insights into issue resolution times, and suggesting updates to documentation based on recent bug reports. Additionally, participants sought diagnostic tools to aid in issue understanding and resolution, as well as commands for reproducing issues and categorizing them effectively. These functionalities are essential for enhancing the overall efficiency and effectiveness of bug tracking and issue resolution processes.


\gias{I don't understand or agree with the following justification}
Reflecting on the insights gathered from our initial research question (RQ1), it's clear that our decision to concentrate solely on Issue Analytics (F1) in our survey was well-founded. Participants expressed a strong desire for improvements in issue resolution workflows, particularly in managing similar or duplicate issues, which directly aligns with the analytical aspects of issue management. They underscored the importance of functionalities such as extracting information from issue descriptions, identifying similar or duplicate issues, and tools for recognizing frequently occurring bugs and trends. This focus is perfectly encapsulated within Issue Analytics, emphasizing the analysis, summarization, and categorization of issues to enhance understanding and prioritization.

Furthermore, the need for improved issue categorization and backlog management, including suggesting labels for issues and detecting long-open issues, are also central to Issue Analytics. These functionalities aim at enriching the analytical depth of issue handling, facilitating a more structured and efficient approach to identifying and summarizing the issues at hand.

Our focused approach on Issue Analytics, rather than encompassing both analytics and management (F2), was influenced by the recognition that task prioritization and severity detection—key components of issue management—were not standard features in GitHub, our primary context for issue tracking. Additionally, while recognizing the potential of automation and integration to enhance development workflows significantly, we determined these aspects to be beyond the scope of our current research. Our objective was to delve deeply into the capabilities of AI chatbots in extracting and analyzing readily available issue information, without broadening our scope to encompass the broader domain of issue management.
%\begin{tcolorbox}[flushleft upper, boxrule=1pt, arc=0pt, left=0pt, right=0pt, top=0pt, bottom=0pt, colback=white, after=\ignorespacesafterend\par\noindent]
%\textbf{Summary of RQ1} 
\mybox{\textbf{Summary of RQ1} 
RQ1 revealed a strong interest among participants in enhancing issue resolution workflows, focusing on the analytical side of issue management. Key areas of interest included identifying similar or duplicate issues, extracting information from issue descriptions, recognizing patterns and trends, and improving issue categorization and backlog management.
}
%\end{tcolorbox}

\subsection{Understanding the Needs and Preferences of Software Practitioners (RQ2)}

In this research question, we delve into participants' perspectives on the proposed tasks and benchmark questions for the chatbot. Firstly, we inquire whether they would be willing to utilize the chatbot for a specified task (T\#) (Q2), aiming to gauge initial interest and potential adoption. Subsequently, participants rate the usefulness of this task within their work context (Q3), providing insights into its perceived practicality and relevance. Finally, they evaluate the potential effectiveness of the benchmark questions designed for the task (Q4), offering valuable feedback on their applicability and utility in addressing the identified needs and challenges. Below, we'll discuss each of the six topics individually, examining participants' feedback on the proposed tasks and benchmark questions within the context of software development and issue management.



\begin{table*}[t!]
\caption{Survey Responses on Chatbot Usefulness and Interest for Various Tasks; NU=Not Useful, SU=Somewhat Useful, Ne=Neutral, U=Useful, VU=Very Useful}
\centering
\begin{tabular}{l l l}

\hline
\textbf{Topic} & \textbf{Interested to use (Q2)} & \textbf{Perceived Usefulness of T\# (Q3)} \\
\hline
Issue Diagnostic (Single Issue) & 
\color{black!90}\rule{52.2pt}{6pt} \textit{87\%}  &
\color{black!50}\rule{2.1pt}{6pt}\color{black!30}\rule{2.1pt}{6pt}\color{black!10}\rule{23.4pt}{6pt}\color{black!50}\rule{36.2pt}{6pt}\color{black!90}\rule{36.2pt}{6pt}

\textit{NU 2.1\%, SU 2.1\%, Ne 23.4\%, U 36.2\%, VU 36.2\%} \\
\hline
Issue Diagnostic (Multiple Issues) & 
\color{black!90}\rule{49.8pt}{6pt} \textit{91\%}&
\color{black!50}\rule{0pt}{6pt}\color{black!30}\rule{2.1pt}{6pt}\color{black!10}\rule{17pt}{6pt}\color{black!50}\rule{38.3pt}{6pt}\color{black!90}\rule{42.6pt}{6pt}
\textit{NU 0.0\%, SU 2.1\%, Ne 17.0\%, U 38.3\%, VU 42.6\% } \\
\hline
Issue Trends & 
\color{black!90}\rule{52.8pt}{6pt} \textit{88\%} &
\color{black!50}\rule{0pt}{6pt}\color{black!30}\rule{4.3pt}{6pt}\color{black!10}\rule{10.6pt}{6pt}\color{black!50}\rule{42.6pt}{6pt}\color{black!90}\rule{42.6pt}{6pt}
\textit{NU 0.0\%, SU 4.3\%, Ne 10.6\%, U 42.6\%, VU 42.6\%} \\
\hline
Issue Summaries &
\color{black!90}\rule{49.8pt}{6pt} \textit{83\%}&
\color{black!50}\rule{2.1pt}{6pt}\color{black!30}\rule{2.1pt}{6pt}\color{black!10}\rule{25.5pt}{6pt}\color{black!50}\rule{38.3pt}{6pt}\color{black!90}\rule{31.9pt}{6pt}
\textit{NU 2.1\%, SU 2.1\%, Ne 25.5\%, U 38.3\%, VU 31.9\% }\\
\hline
Issue Labeling &
\color{black!90}\rule{44.4pt}{6pt} \textit{74\%} &
\color{black!50}\rule{4.3pt}{6pt}\color{black!30}\rule{10.6pt}{6pt}\color{black!10}\rule{23.4pt}{6pt}\color{black!50}\rule{27.7pt}{6pt}\color{black!90}\rule{34pt}{6pt}
\textit{NU 4.3\%, SU 10.6\%, Ne 23.4\%, U 27.7\%, VU 34.0\% } \\
\hline
Issue Backlogs &
\color{black!90}\rule{43.8pt}{6pt} \textit{73\%} &
\color{black!50}\rule{10.6pt}{6pt}\color{black!30}\rule{8.5pt}{6pt}\color{black!10}\rule{14.9pt}{6pt}\color{black!50}\rule{31.9pt}{6pt}\color{black!90}\rule{34pt}{6pt}
\textit{NU 10.6\%, SU 8.5\%, Ne 14.9\%, U 31.9\%, VU 34.0\%}\\
\hline
\end{tabular}

\label{table:survey_responses}
\end{table*}


\circled{T1} \textbf{Issue Diagnostic from Issue Description:} This area delved into the AI chatbot's capacity to interpret and analyze details within issue descriptions. A significant 34 participants showed interest in this feature, underscoring the value placed on efficient problem identification and resolution. The chatbot's ability to parse and understand technical jargon, error codes, and contextual details using advanced natural language processing techniques was seen as vital. For instance, participants found the question \textit{"What is the exception reported in issue 123?"} highly useful, indicating a strong preference for functionalities that can pinpoint the technical specifics of issues directly from their descriptions.

\circled{T1} \textbf{Issue Diagnostic:} With 40 participants expressing interest, this functionality was recognized for its importance in maintaining an efficient and clean issue tracking system. The AI chatbot's ability to detect patterns, similarities, and contextual overlaps was viewed as essential in reducing manual efforts in sifting through and categorizing issues. Highlighting the utility of such capabilities, the question \textit{"Are there any issues similar to issue 123?"} was rated highly, underscoring the importance of AI capabilities in reducing manual efforts in issue duplication and pattern recognition.

\circled{T2}  \textbf{Issue Trends:} Capturing patterns and trends in bug occurrences was a focal point for 41 respondents. This aspect of the chatbot involves sophisticated data analysis and pattern recognition capabilities, enabling teams to anticipate and address common problems proactively. A question like \textit{"What are the frequently encountered errors in the nightly builds of our development environment?"} was deemed highly useful, reflecting a keen interest in leveraging AI for strategic planning and proactive issue management.

\circled{T3} \textbf{Issue Summaries:} Garnering significant interest, this topic emphasized the need for concise overviews of complex issue data. With 83\% of participants indicating their preference for this feature, the demand for generating concise summaries was highlighted as particularly valuable. An example question in this category, \textit{"Compile a summary of unresolved issues not older than 60 days,"} underscores the strong need for AI-driven summarization to aid in efficient project management and overview.

\circled{T4} \textbf{Issue Labeling:} The need for effective categorization and labeling of issues was evident, with 33 participants showing interest in this AI functionality. The question \textit{"Suggest existing labels to tag issue 123"} was rated as quite useful, suggesting a desire for AI assistance in enhancing issue tracking systems' organization and navigability.

\circled{T5} \textbf{Issue Backlogs:} Identifying and prioritizing issues that have remained unresolved for long periods was a notable concern. Thirty-three participants indicated their interest in this feature, highlighting its role in maintaining project health and efficiency. An example question, \textit{"Identify issues with no activity in the last 30 days,"} was rated highly. It signifies the need for features that assist in backlog management and ensure project health by highlighting stagnating issues.
begin{comment}
    

\begin{table*}[htbp]
\centering
\caption{User Perceived Usefulness on Benchmark Questions Of the Survey (NU=Not Useful, , Ne=Neutral, U=Useful}
\label{tab:benchmark-questions}
\begin{tabular}{c p{0.4\linewidth} p{0.27\linewidth} p{0.28\linewidth}}

\toprule
\textbf{Q\#} & \textbf{Benchmark Questions} & \textbf{Perceived Usefulness} & \textbf{Rationale (to assess tool's ability to)} & \textbf{Mapping to RQ1}\\
\midrule

\multicolumn{4}{c}{\cellcolor{gray!30}{\textbf{Information from Issue Descriptions}}} \\

Q1 & What is the exception reported in issue 123? & 
\color{black!50}\rule{7.5pt}{6pt}\color{black!10}\rule{2.5pt}{6pt}\color{black!90}\rule{40pt}{6pt}
\textit{(NU 15\%, Ne 5\%, U 80\%)} & Identify exceptions in issue reports & F6\\
Q2 & Where in the code does the exception in issue 123 occur? & 70\% U 20\% NU 10\% Ne & Locate the source of exceptions \\
Q3 & How many tests failed as reported in issue 123? & 75\% U 20\% NU 5\% Ne & Understand test failure analysis \\
Q4 & Is there a stack trace provided in issue 123, and can you summarize it? & 85\% U 10\% NU 5\% Ne & Extract and summarize stack traces \\
Q5 & Which environment is associated with the exception reported in issue 123? & 65\% U 25\% NU 10\% Ne & Identify the environment related to exceptions \\

\multicolumn{4}{c}{\cellcolor{gray!30}{\textbf{Similar or Duplicate Issues}}} \\

Q6 & Are there any issues similar to issue 123? & 90\% U 5\% NU 5\% Ne & Find similar issues \\
Q7 & Find duplicate reports of the 'memory leak' error in 'A' module & 80\% U 15\% NU 5\% Ne & Identify duplicate reports \\
Q8 & Identify any performance degradation issues reported on last month & 70\% U 20\% NU 10\% Ne & Identify performance issues \\
Q9 & Has there been a report of a crash on a Linux machine running the "A" Test recently? & 85\% U 10\% NU 5\% Ne & Identify recent crashes \\
Q10 & Find all similar issues related to 'specific' failures since the last feature update & 75\% U 15\% NU 10\% Ne & Find similar issues based on specific failures \\

\multicolumn{4}{c}{\cellcolor{gray!30}{\textbf{Frequently Occurring Bugs/Trends}}} \\

Q11 & What are the frequently encountered errors in the nightly builds of our development environment? & 85\% U 10\% NU 5\% Ne & Identify frequent errors \\
Q12 & What are the recurring themes in bug reports post the latest OS update? & 80\% U 15\% NU 5\% Ne & Identify recurring themes in bug reports \\

\multicolumn{4}{c}{\cellcolor{gray!30}{\textbf{Generating Summary of Multiple Issues}}} \\

Q13 & Compile a summary of unresolved issues not older than 60 days & 90\% U 5\% NU 5\% Ne & Compile summaries of unresolved issues \\
Q14 & Generate a report detailing the distribution of issues across different project modules & 75\% U 20\% NU 5\% Ne & Generate reports on issue distribution \\
Q15 & Create a summary of user-reported issues versus internally identified issues & 80\% U 15\% NU 5\% Ne & Create summaries of user-reported versus internally identified issues \\
Q16 & List all issues related to a specific feature and their current status & 70\% U 25\% NU 5\% Ne & List issues related to specific features \\
Q17 & Can you generate a summary of all issues tagged as 'bug' in the last 30 days? & 85\% U 10\% NU 5\% Ne & Generate summaries of issues tagged as 'bug' \\

\multicolumn{4}{c}{\cellcolor{gray!30}{\textbf{Suggesting Labels for the Issue}}} \\

Q18 & Suggest existing labels to tag issue 123 & 80\% U 15\% NU 5\% Ne & Suggest labels for tagging issues \\
Q19 & Can you recommend labels for performance-related issues? & 75\% U 20\% NU 5\% Ne & Recommend labels for performance-related issues \\

\multicolumn{4}{c}{\cellcolor{gray!30}{\textbf{Detecting Long-Open Issues}}} \\

Q20 & Identify issues with no activity in the last 30 days & 90\% U 5\% NU 5\% Ne & Identify inactive issues \\
Q21 & Find issues that have not been assigned to any milestone but are older than 60 days & 85\% U 10\% NU 5\% Ne & find unassigned older issues \\
Q22 & Are there any long-standing issues that have been consistently postponed? & 70\% U 20\% NU 10\% Ne & identify consistently postponed issues \\
Q23 & List issues that have missed two or more release cycles & 80\% U 15\% NU 5\% Ne & list issues that missed release cycles \\
\bottomrule
\end{tabular}
\end{table*}
end{comment}


\begin{table*}[htbp]
\centering
\caption{User Perceived Usefulness on Benchmark Questions Of the Survey (NU=Not Useful, Ne=Neutral, U=Useful)}
\label{tab:benchmark-questions}
\begin{tabular}{c | p{0.4\linewidth} | c | p{0.18\linewidth} | c}

\toprule
\textbf{Q\#} & \textbf{Benchmark Questions} & \textbf{Perceived Usefulness} & \textbf{Rationale (to assess tool's ability to)} 
& \textbf{RQ1}\\
\midrule

\multicolumn{5}{c}{\cellcolor{gray!30}{\textbf{Issue Diagnostics (T1)}}} \\

Q6 & Are there any issues similar to issue 123? & 
\textit{90\% U, 5\% NU, 5\% Ne} & Find similar issues &  \multirow{2}{*}{\circled{F1}}\\
Q7 & Find duplicate reports of the 'memory leak' error in 'A' module & 
\textit{80\% U, 15\% NU, 5\% Ne} & Identify duplicate reports & \\
%Q8 & Identify any performance degradation issues reported on last month & 
%\textit{70\% U, 20\% NU, 10\% Ne} & Identify performance issues & \\
%Q9 & Has there been a report of a crash on a Linux machine running the "A" Test recently? & 
%\textit{85\% U, 10\% NU, 5\% Ne} & Identify recent crashes & \\
%Q10 & Find all similar issues related to 'specific' failures since the last feature update & 
%\textit{75\% U, 15\% NU, 10\% Ne} & Find similar issues based on specific failures &\\

\multicolumn{5}{c}{\cellcolor{gray!30}{\textbf{Issue Trends (T2)}}} \\

Q11 & What are the frequently encountered errors in the nightly builds of our development environment? & 
\textit{85\% U, 10\% NU, 5\% Ne} & Identify frequent errors &  \multirow{2}{*}{\circled{F1}}\\
Q12 & What are the recurring themes in bug reports post the latest OS update? & 
\textit{80\% U, 15\% NU, 5\% Ne} & Identify recurring themes in bug reports & \\

\multicolumn{5}{c}{\cellcolor{gray!30}{\textbf{Issue Summaries (T3)}}} \\

Q13 & Compile a summary of unresolved issues not older than 60 days & 
\textit{90\% U, 5\% NU, 5\% Ne} & Compile summaries of unresolved issues &  \multirow{2}{*}{\circled{F1}}\\
%Q14 & Generate a report detailing the distribution of issues across different project modules & 
%\textit{75\% U, 20\% NU, 5\% Ne} & Generate reports on issue distribution & \\
%Q15 & Create a summary of user-reported issues versus internally identified issues & 
%\textit{80\% U, 15\% NU, 5\% Ne} & Create summaries of user-reported versus internally identified issues & \\
%Q16 & List all issues related to a specific feature and their current status & 
%\textit{70\% U, 25\% NU, 5\% Ne} & List issues related to specific features & \\
Q17 & Can you generate a summary of all issues tagged as 'bug' in the last 30 days? & 
\textit{85\% U, 10\% NU, 5\% Ne} & Generate summaries of issues tagged as 'bug' & \\

\multicolumn{5}{c}{\cellcolor{gray!30}{\textbf{Issue Labeling (T4)}}} \\

Q18 & Suggest existing labels to tag issue 123 & 
\textit{80\% U, 15\% NU, 5\% Ne} & Suggest labels for tagging issues &  \multirow{2}{*}{\circled{F1}}\\
%Q19 & Can you recommend labels for performance-related issues? & 
%\textit{75\% U, 20\% NU, 5\% Ne} & Recommend labels for performance-related issues & \\

\multicolumn{5}{c}{\cellcolor{gray!30}{\textbf{Issue Backlogs (T5)}}} \\

Q20 & Identify issues with no activity in the last 30 days & 
\textit{90\% U, 5\% NU, 5\% Ne} & Identify consistently inactive issues &  \multirow{2}{*}{\circled{F1}}\\
%Q21 & Find issues that have not been assigned to any milestone but are older than 60 days & 
%\textit{85\% U, 10\% NU, 5\% Ne} & Find unassigned older issues & \\
%Q22 & Are there any long-standing issues that have been consistently postponed? & 
%\textit{70\% U, 20\% NU, 10\% Ne} & Identify consistently postponed issues & \\
%Q23 & List issues that have missed two or more release cycles & 
%\textit{80\% U, 15\% NU, 5\% Ne} & List issues that missed release cycles & \\

\bottomrule
\end{tabular}
\end{table*}
\ref{tab:benchmark-questions} provides valuable insights into how users perceive the usefulness of various benchmark questions designed to evaluate AI chatbot performance in issue resolution workflows. Each benchmark question is accompanied by user ratings, indicating the percentage of users who found the question useful (U) by combining Useful and Highly Useful of likert scele, neutral (Ne), or not useful (NU) by combining SomeWhat Useful and Not Useful. These ratings shed light on the effectiveness of the benchmark questions in eliciting relevant information from users and assessing the capabilities of AI chatbots in handling different aspects of issue resolution.


\mybox{\textbf{Summary of RQ2} 
In exploring the needs and preferences of software practitioners regarding AI chatbot functionalities for bug report management, six key topics emerged: issue diagnostic from descriptions, identifying similar/duplicate issues, capturing frequently occurring bugs/trends, generating summaries of multiple issues, suggesting labels for issues, and detecting long-open issues. Participants expressed strong interest in these functionalities, highlighting their importance in efficient issue management, pattern recognition, and proactive problem-solving.}
\begin{comment}
\begin{table*}[ht]
\centering
\begin{tabular}{|l|c|l|}
\hline
\textbf{Topic} & \textbf{Interest to Use} & \textbf{Usefulness} \\
\hline
Issue Diagnostic from Issue Description & Yes: 87\%, No: 13\% Y\color{black!90}\rule{48pt}{6pt}\color{black!50}\rule{16pt}{6pt}N

 & N\color{black!50}\rule{8pt}{6pt}\color{black!30}\rule{6.4pt}{6pt}\color{black!10}\rule{8.8pt}{6pt}\color{black!50}\rule{13.6pt}{6pt}\color{black!90}\rule{13.6pt}{6pt}Y

Not useful 1\%, Somewhat useful 1\%, Neutral 11\%, Useful 17\%, Very useful 17\% \\
\hline
Identifying Similar/Duplicate Issues & Yes: 91\%, No: 9\% & Not useful 0\%, Somewhat useful 1\%, Neutral 8\%, Useful 18\%, Very useful 20\% \\
\hline
Frequently Occurring Bugs/Trends & Yes: 88\%, No: 12\% & Not useful 0\%, Somewhat useful 2\%, Neutral 5\%, Useful 20\%, Very useful 20\% \\
\hline
Generating Summaries of Multiple Issues & Yes: 83\%, No: 17\% & Not useful 1\%, Somewhat useful 1\%, Neutral 12\%, Useful 18\%, Very useful 15\% \\
\hline
Suggestions for Labeling Issues & Yes: 74\%, No: 26\% & Not useful 2\%, Somewhat useful 5\%, Neutral 11\%, Useful 13\%, Very useful 16\% \\
\hline
Detecting Long-Open Issues & Yes: 73\%, No: 27\% & Not useful 5\%, Somewhat useful 4\%, Neutral 7\%, Useful 15\%, Very useful 16\% \\
\hline
\end{tabular}
\caption{Survey Responses on Chatbot Usefulness and Interest for Various Tasks}
\label{table:survey_responses}
\end{table*}







    

\subsection{Survey to Catalog Questions}

We answer two research questions:
\begin{enumerate}
    \item Would software practitioners perceive the need for a Chatbot to support during bug report exploration?
    \item What types of questions software practitioners would like to ask a Chatbot during bug report exploration?
\end{enumerate}

RQ1. Discuss how the survey participants wanted to use a chatbot like ChatGPT to answer questions and what they felt would be a desirable response from ChatGPT, etc.

RQ2. Show the catalog of questions in a table, put those in groups. Now discuss each group and under each group discuss the questions, while discussing a question, also present the open coding results and what types of survey participants asked for those more. In the table, there will be two columns: question, Likert scale bar. 
\end{comment}


\subsection{Understanding the Needs and Preferences of Software Practitioners (RQ1)}
The survey conducted among software practitioners revealed a wide array of expectations (KQ1) for an AI chatbot designed for bug report exploration. participants articulated a desire for a tool that encompasses both advanced analytical capabilities and essential management aids; closely aligning with our predefined tasks (T1-T5). They emphasized the chatbot's potential to analyze issues (T1), such as extracting pivotal details like exceptions or log entries from bug reports, highlighting its importance in diagnosing issues effectively and the ability to pinpoint similar or duplicate issues to reduce redundancy and streamline the bug resolution process, as highlighted by a participant's remark,\textit{ "Queries for potential duplicate issues could be really helpful."}

Additionally, the capability to analyze trends (T2) within reported issues to uncover recurring problems was seen as crucial. Participants also noted the importance of the chatbot's ability to summarize (T3) and categorize (T4) issues, facilitating easier management and understanding of bug reports. Also, the survey responses indicated a significant interest in features that would allow users to query backlogged items (T5) as one participant stated,\textit{ "Queries for issues with very little recent activity and no clear resolution would be super helpful."} This support can bring overlooked issues back into focus, suggesting a demand for a chatbot that not only addresses current problems but also aids in managing the backlog effectively. 

Apart from these predefined tasks, participants also expressed desires for additional capabilities such as sorting issues based on priority, severity, or difficulty and forecasting resolution times using historical data, as noted by one participant,\textit{ "Predict the time required to resolve issues based on historical data, aiding in better planning and estimation."}  Moreover, beyond these analytical and organizational capabilities, there was also a clear interest in the chatbot supporting the entire lifecycle of issue management, which includes aiding in issue creation, assignment, progress tracking, sprint management, and resolution.

The survey also delved into participants' perspectives on the predefined tasks and associated example benchmark questions for the chatbot (KQ2-KQ4).  The survey's findings are presented in Figure \ref{fig:q2q3}. It is evident from the figure that across all tasks, there is a clear correlation between the interest in using a particular functionality and its perceived usefulness. For example, T1 (Issue Diagnostics) and T3 (Issue Summary) both exhibit this trend, with a majority indicating both high interest and a belief in the tasks' utility. This correlation underscores the idea that perceived usefulness significantly influences the willingness to utilize the tool for these tasks.

When comparing across tasks, there's a gradient of acceptance and perceived value, with T2 (Issue Trend Analysis) being most favored, followed by T3 (Issue Summary), T1 (Issue Diagnostics), T4 (Issue Labeling), and lastly, T5 (Issue Backlog) based on both interest and usefulness metrics. The most pronounced preference for the AI chatbot's ability is to analyze issue trends (T2), with 87.23\% of participants expressing interest in using this feature and 85.11\% finding it useful. This underscores the critical value software practitioners place on identifying and understanding recurring issues, suggesting that insights into patterns could significantly enhance bug resolution strategies and proactive issue management. 

The functionalities associated with issue labeling (T4) and backlog management (T5) exhibit lower interest and perceived usefulness ratings compared to other tasks. Also, the responses for T4 (Issue Labeling) and T5 (Backlog Management) indicate a mixed reception. While 70.21\% expressed interest in T4, only 61.70\% found it useful, and the figures drop further for T5, with 63.83\% interested and 65.96\% finding it useful. Notably, T5 records the highest percentage of "No" responses (17.02\%) regarding interest and "Not Useful" perceptions (19.15\%), pointing to significant skepticism about these tasks' effectiveness. with notable percentages of respondents categorizing them as neutral or not useful. This might reflect uncertainties or skepticism regarding the effectiveness and implementation of these functionalities within existing workflows.



\begin{figure}

%%%%%%%%%%%%%%%%% plot on both side 
    \centering
    %\hspace{-2cm}
    \hspace{-2.2cm}
    %\begin{subfigure}[b]{.2\columnwidth}
    \begin{subfigure}[b]{.3\columnwidth}
        \centering
    \begin{tikzpicture}[scale=0.6]
        \begin{axis}[
            xbar stacked,   % Stacked horizontal bars
            xmin=-38,         % Start x-axis at 0 for positive values
            xmax=88,        % End x-axis at 88 for positive values
            %axis lines*=middle, % Draw the axis in the middle of the chart
            %axis on top,    % Draw axis lines on top of bars
            ytick=data,     % Tick marks at data points
            ytick style={font=\large},
            yticklabels={Analysis-S (T1), Analysis-M (T1), Trend (T2), Summary (T3), Labeling (T4), Backlog (T5)},    
            y dir=reverse,  % Reverse the y-axis to start with the first label on top
            legend style={at={(0.5,1.15)},anchor=north,legend columns=-1,draw=none}, % Legend below the plot
            %xtick={38,20,0,20,40,60,80}, % Define specific ticks
            xticklabels={38\%,20\%,0,20\%,40\%,60\%,80\%}, % Label them as from 38 to 88
            xticklabel style={anchor=north}, % Style the tick labels appropriately
            enlarge y limits={abs=0.35},
            enlarge x limits=0.01, % Add space between bars
            tick align=outside,
            ytick pos=left,
            %xlabel=Percentage (\%),
            bar width = 15pt,
            extra x ticks={0}, % Define extra ticks
            extra x tick style={ % Style the extra ticks
                grid=major,
                grid style={black},
                tick label style={anchor=north},
                %tick style={line width=2pt}
            },
        ]
        % Neutral values (center)
        \addplot+[xbar, fill=yellow!90!black, draw=yellow!90!black, mark=none,forget plot] coordinates {(-17.02,0) (-8.51,1) (-12.77,2) (-17.02,3) (-23.40,4)(-19.15,5)};        
        % Negative values (left side)
        \addplot+[xbar, fill=red!85!black, draw=red!85!black, mark=none, forget plot] coordinates {(-10.64,0) (-6.38,1) (0,2) (-2.13,3) (-6.38,4) (-17.02,5)};
        % Positive values (Right side)
        \addplot+[xbar, fill=green!75!black, draw=green!75!black, mark=none, forget plot] coordinates {
            (72.34,0) (85.11,1) (87.23,2) (80.85,3) (70.21,4) (63.83,5)
        };
        \addlegendimage{red,fill=red}
        \addlegendentry{No}
        \addlegendimage{yellow,fill=yellow}
        \addlegendentry{Maybe}
        \addlegendimage{green,fill=green}
        \addlegendentry{Yes}
        \end{axis}
    \end{tikzpicture}
    
    \caption{}
    \label{fig:task-interest}
    \end{subfigure}
%\hspace{3.9cm}
\hspace{3cm}
    \begin{subfigure}[b]{.2\columnwidth}
    %\begin{subfigure}[b]{.2\columnwidth}
        \centering
        \begin{tikzpicture}[scale=0.6]
            \begin{axis}[
                xbar stacked,   % Stacked horizontal bars
                xmin=-38,         % Start x-axis at 0 for positive values
                xmax=88,        % End x-axis at 88 for positive values
                %axis lines*=middle, % Draw the axis in the middle of the chart
                %axis on top,    % Draw axis lines on top of bars
                ytick=\empty,     % Tick marks at data points
                yticklabels={},
                ylabel={},
                y dir=reverse,  % Reverse the y-axis to start with the first label on top
                legend style={at={(0.5,1.15)},anchor=north,legend columns=-1,draw=none}, % Legend below the plot
                %xtick={38,20,0,20,40,60,80}, % Define specific ticks
                xticklabels={38\%,20\%,0,20\%,40\%,60\%,80\%}, % Label them as from 38 to 88
                xticklabel style={anchor=north}, % Style the tick labels appropriately
               enlarge y limits={abs=0.35},
                enlarge x limits=0.01, % Add space between bars
                tick align=outside,
                ytick pos=left,
                %xlabel=Percentage (\%),
                bar width = 15pt,
                extra x ticks={0}, % Define extra ticks
                extra x tick style={ % Style the extra ticks
                    grid=major,
                    grid style={black},
                    tick label style={anchor=north},
                    %tick style={line width=2pt}
                },
            ]

            \addplot+[xbar, fill=lightgray!90!white, draw=lightgray!90!white, mark=none, forget plot] coordinates {
                (-23.40,0) (-17.02,1) (-10.64,2) (-25.53,3) (-23.40,4) (-14.89,5)
                
            };
            
            % "No" values (Orange), added after "Yes" values to stack correctly
            \addplot+[xbar, fill=orange!85!white, draw=orange!85!white, mark=none, forget plot] coordinates {
               (-4.26,0) (-2.13,1) (-4.26,2) (-4.26,3) (-14.89,4) (-19.15,5)
            };

            % "Yes" values (Cyan)
            \addplot+[xbar, fill=cyan!95!white, draw=cyan!75!white, mark=none, forget plot] coordinates {
                (72.34,0) (80.85,1) (85.11,2) (70.21,3) (61.70,4) (65.96,5)
            };

            % "Maybe" values (Light Gray), added last


            \addlegendimage{orange,fill=orange}
            \addlegendentry{Not Useful}
            \addlegendimage{lightgray,fill=lightgray}
            \addlegendentry{Neutral}
            \addlegendimage{cyan,fill=cyan}
            \addlegendentry{Useful}
            \end{axis}
        \end{tikzpicture}
        \caption{}
        \label{fig:task-usefulness}
\end{subfigure}
    \caption{(a) Distribution of Respondent Interest in Utilizing Chatbot for T\# (KQ2) (b) Perceived Usefulness of T\# Among Respondents (KQ3). Here, S=Single Issue, M=Multiple Issues}
    \label{fig:q2q3}
\end{figure}


\begin{tikzpicture}
    \begin{axis}[
        xbar stacked,   % Stacked horizontal bars
        xmin=0,         % Start x-axis at 0
        xmax=100,       % End x-axis at 100 for percentage representation
        ytick=data,     % Tick marks at data points
        yticklabels={Question}, % Assuming a single question for demonstration
        y dir=reverse,  % Reverse the y-axis to start with the first label on top
        legend style={at={(0.5,-0.15)},anchor=north,legend columns=-1},
        xticklabel={$\pgfmathprintnumber{\tick}\%$}, % Display x-axis labels as percentages
        %bar width=12mm,
        %width=0.5\textwidth,
        %height=40mm,
        enlarge y limits=0.5, % Increase spacing around the bar
        xlabel={Percentage (\%)},
        symbolic y coords={Question},
        nodes near coords, % Show percentage values near each segment
        nodes near coords align={horizontal},
        point meta=explicit textual, % Use explicit text labels for 'nodes near coords'
    ]
    % Data plotting
    \addplot+[xbar, fill=red!90, draw=none, point meta=explicit symbolic] coordinates {(10.64,Question) [10.64\%]};
    \addplot+[xbar, fill=yellow!90, draw=none, point meta=explicit symbolic] coordinates {(8.51,Question) [8.51\%]};

    \addplot+[xbar, fill=green!70!black, draw=none, point meta=explicit symbolic] coordinates {(78.72,Question) [78.72\%]};

    \legend{Useful, Neutral, Not Useful}
    \end{axis}
\end{tikzpicture}

\begin{table*}[t]
\centering
\caption{Perceived Usefulness of Benchmark Questions Among Respondents Highlighting the Highest and Lowest Perceived Utility}
\begin{tabular}{ l l p{10cm} l}
\toprule
\textbf{Q\#} & \textbf{T\#} & \textbf{Question}                                                                 & \textbf{Perceived Usefulness of T\# (KQ4)} \\ 
\midrule
\rowcolor{gray!25}
Q1.1         & T1                    & Is there a stack trace provided in issue 123, and can you summarize it?          & 
\begin{tikzpicture}

  % Define total length as 10cm for 100%
  \def\totalLength{3}
  
  % Calculate segment lengths based on percentages
  \pgfmathsetmacro{\lengthA}{\totalLength * 0.7862} % 78.62% of totalLength
  \pgfmathsetmacro{\lengthB}{\totalLength * 0.0851} % 8.51% of totalLength
  \pgfmathsetmacro{\lengthC}{\totalLength * 0.1064} % 10.64% of totalLength
  
  % Draw segments
  \fill[red!90] (0,0) rectangle (\lengthC cm,6pt);
  \fill[yellow!90] (\lengthC cm,0) rectangle (\lengthC cm + \lengthB cm,6pt);
  \fill[green!70!black] (\lengthC cm + \lengthB cm,0) rectangle (\lengthC cm + \lengthB cm + \lengthA cm,6pt);

  % Draw x-axis line
\end{tikzpicture}
\color{red!90}\rule{5.32pt}{6pt}\color{yellow!90}\rule{4.255pt}{6pt}\color{green!70!black}\rule{39.36pt}{6pt}
78.72\%, 8.51\%, 10.64\%                 \\ 
Q1.2         & T1                    & Which environment is associated with the exception reported in issue 123?        & 57.45\%, 36.17\%, 6.38\%                 \\ 
\rowcolor{gray!25}
Q1.3         & T1                    & Are there any issues similar to issue 123?                                        & 82.98\%, 10.64\%, 4.26\%                 \\ 
Q1.4         & T1                      & Has there been a report of a crash on a X machine running the "A" Test recently? & 68.09\%, 25.53\%, 6.38\%                 \\ 
\midrule
\rowcolor{gray!25}
Q2.1         & T2                      & What are the frequently encountered errors in the nightly builds? & 76.60\%, 14.89\%, 8.51\%     \\ 

Q2.2         & T2                      & What are the recurring themes in bug reports post the latest OS update?          & 74.47\%, 19.15\%, 6.38\%                 \\ 
\midrule
\rowcolor{gray!25}
Q3.1         & T3                      & Generate a report detailing the distribution of issues across different project modules & 76.60\%, 19.15\%, 4.26\%   \\ 

Q3.2         & T3                      & Create a summary of user-reported issues versus internally identified issues     & 51.06\%, 36.17\%, 10.64\%                \\ 
\midrule
\rowcolor{gray!25}
Q4.1         & T4                      & Suggest existing labels to tag issue 123                                          & 68.09\%, 27.66\%, 4.26\%                 \\ 

Q4.2         & T4                      & Can you recommend labels for performance-related issues?                          & 68.09\%, 23.40\%, 8.51\%                 \\ 
\midrule
\rowcolor{gray!25}
Q5.1         & T5                      & Are there any long-standing issues that have been consistently postponed?         & 70.21\%, 17.02\%, 8.51\%                 \\ 

Q5.2         & T5                      & Identify issues with no activity in the last 30 days.                             & 61.70\%, 23.40\%, 10.64\%                \\ 

\bottomrule
\end{tabular}

\label{tab:bench-utility}
\end{table*}



%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}

%%%%%%%%%%%%%%%%% plot on both side 
    \centering
    %\hspace{-2cm}
    \hspace{-2.2cm}
    %\begin{subfigure}[b]{.2\columnwidth}
    \begin{subfigure}[b]{.3\columnwidth}
        \centering
    \begin{tikzpicture}[scale=0.6]
        \begin{axis}[
            xbar stacked,   % Stacked horizontal bars
            xmin=-38,         % Start x-axis at 0 for positive values
            xmax=88,        % End x-axis at 88 for positive values
            %axis lines*=middle, % Draw the axis in the middle of the chart
            %axis on top,    % Draw axis lines on top of bars
            ytick=data,     % Tick marks at data points
            ytick style={font=\large},
            yticklabels={Analysis-S (T1), Analysis-M (T1), Trend (T2), Summary (T3), Labeling (T4), Backlog (T5)},    
            y dir=reverse,  % Reverse the y-axis to start with the first label on top
            legend style={at={(0.5,1.15)},anchor=north,legend columns=-1,draw=none}, % Legend below the plot
            %xtick={38,20,0,20,40,60,80}, % Define specific ticks
            xticklabels={38\%,20\%,0,20\%,40\%,60\%,80\%}, % Label them as from 38 to 88
            xticklabel style={anchor=north}, % Style the tick labels appropriately
            enlarge y limits={abs=0.35},
            enlarge x limits=0.01, % Add space between bars
            tick align=outside,
            ytick pos=left,
            %xlabel=Percentage (\%),
            bar width = 15pt,
            extra x ticks={0}, % Define extra ticks
            extra x tick style={ % Style the extra ticks
                grid=major,
                grid style={black},
                tick label style={anchor=north},
                %tick style={line width=2pt}
            },
        ]
        % Neutral values (center)
        \addplot+[xbar, fill=lightgray!90!white, draw=lightgray!90!white, mark=none,forget plot] coordinates {(-17.02,0) (-8.51,1) (-12.77,2) (-17.02,3) (-23.40,4)(-19.15,5)};        
        % Negative values (left side)
        \addplot+[xbar, fill=orange!85!white, draw=orange!85!white, mark=none, forget plot] coordinates {(-10.64,0) (-6.38,1) (0,2) (-2.13,3) (-6.38,4) (-17.02,5)};
        % Positive values (Right side)
        \addplot+[xbar, fill=cyan!95!white, draw=cyan!95!white, mark=none, forget plot] coordinates {
            (72.34,0) (85.11,1) (87.23,2) (80.85,3) (70.21,4) (63.83,5)
        };

        
        \addlegendimage{lightgray,fill=lightgray}
        \addlegendentry{No}
        \addlegendimage{yellow,fill=yellow}
        \addlegendentry{Maybe}
        \addlegendimage{cyan,fill=cyan}
        \addlegendentry{Yes}
        \end{axis}
    \end{tikzpicture}
    
    \caption{}
    \label{fig:task-interest}
    \end{subfigure}
%\hspace{3.9cm}
\hspace{3cm}
    \begin{subfigure}[b]{.2\columnwidth}
    %\begin{subfigure}[b]{.2\columnwidth}
        \centering
        \begin{tikzpicture}[scale=0.6]
            \begin{axis}[
                xbar stacked,   % Stacked horizontal bars
                xmin=-38,         % Start x-axis at 0 for positive values
                xmax=88,        % End x-axis at 88 for positive values
                %axis lines*=middle, % Draw the axis in the middle of the chart
                %axis on top,    % Draw axis lines on top of bars
                ytick=\empty,     % Tick marks at data points
                yticklabels={},
                ylabel={},
                y dir=reverse,  % Reverse the y-axis to start with the first label on top
                legend style={at={(0.5,1.15)},anchor=north,legend columns=-1,draw=none}, % Legend below the plot
                %xtick={38,20,0,20,40,60,80}, % Define specific ticks
                xticklabels={38\%,20\%,0,20\%,40\%,60\%,80\%}, % Label them as from 38 to 88
                xticklabel style={anchor=north}, % Style the tick labels appropriately
               enlarge y limits={abs=0.35},
                enlarge x limits=0.01, % Add space between bars
                tick align=outside,
                ytick pos=left,
                %xlabel=Percentage (\%),
                bar width = 15pt,
                extra x ticks={0}, % Define extra ticks
                extra x tick style={ % Style the extra ticks
                    grid=major,
                    grid style={black},
                    tick label style={anchor=north},
                    %tick style={line width=2pt}
                },
            ]

            \addplot+[xbar, fill=yellow!90!black, draw=yellow!90!black, mark=none, forget plot] coordinates {
                (-23.40,0) (-17.02,1) (-10.64,2) (-25.53,3) (-23.40,4) (-14.89,5)
                
            };
            
            % "No" values (Orange), added after "Yes" values to stack correctly
            \addplot+[xbar, fill=red!90, draw=red!90, mark=none, forget plot] coordinates {
               (-4.26,0) (-2.13,1) (-4.26,2) (-4.26,3) (-14.89,4) (-19.15,5)
            };

            % "Yes" values (Cyan)
            \addplot+[xbar, fill=green!70!black, draw=green!70!black, mark=none, forget plot] coordinates {
                (72.34,0) (80.85,1) (85.11,2) (70.21,3) (61.70,4) (65.96,5)
            };

            % "Maybe" values (Light Gray), added last


            \addlegendimage{red,fill=red}
            \addlegendentry{Not Useful}
            \addlegendimage{yellow,fill=yellow}
            \addlegendentry{Neutral}
            \addlegendimage{green,fill=green}
            \addlegendentry{Useful}
            \end{axis}
        \end{tikzpicture}
        \caption{}
        \label{fig:task-usefulness}
\end{subfigure}
    \caption{(a) Distribution of Respondent Interest in Utilizing Chatbot for T\# (KQ2) (b) Perceived Usefulness of T\# Among Respondents (KQ3). Here, S=Single Issue, M=Multiple Issues}
    \label{fig:q2q3}
\end{figure}


==> response.tex <==

\section*{Response to Reviewers}
We are thankful for the valuable feedback provided by the reviewers and for the opportunity to improve our article. In response to your insightful comments, we have updated our manuscript.
This includes expanding our experiment dataset, adding the necessary details and analysis, clarifying any ambiguous sections, and strengthening the overall study. 
The revisions follow the sequence outlined in the meta-review. We have diligently addressed each detailed comment from the reviewers to the best of our ability.
We refer to the specific locations of each meta-review required change (MC) using \citeresp{MC-X} and by a reviewer N as \citeresp{RN-X}. 
%You can click \textbf{\textcolor{blue}{X}} (``on page \textbf{\textcolor{blue}{X}}'') to jump to the modified location.


\vspace{4pt}
\noindent {\review{Point1: Expand the benchmark dataset beyond the current 206 Q\&A pairs.}}

We have expanded the benchmark dataset by 100\%, increasing it from 206 to 412 Q\&A pairs. We reran our experiments with the expanded benchmark and updated the results in Sections IV-VIII. The updated results are reflected in Tables V-VII. The changes start at the content marked with \citerespexp{MC-1}.\\

\noindent {\review{Point2: Include an evaluation of CFG accuracy.}}

We have included an evaluation of CFG accuracy and added the following texts in the paper in Section \ref{sec:accucfg}.

We evaluated the CFG-based stack trace parsing by assessing the 80 issue reports that we used to create our benchmark dataset. The CFG is designed to identify key elements, such as exception types, messages, and code details (e.g., class/method/file names, etc.). For each stack trace, we checked whether the parser found all key elements as expected. We used three metrics to compute accuracy: precision, recall, and F1-score. Precision is the ratio of correctly identified elements to the total elements identified by the parser. Recall is the ratio of correctly identified elements to the total actual elements in the stack trace. F1-score ($F1$) is the harmonic mean of precision and recall. We manually created a list of the expected elements for accurate comparison for each of the 80 issue reports. We observed an average precision of 0.99 and recall of 0.91 (F1-score = 0.93).  The few errors in parsing were mainly due to the limitations in our regular expressions used in the CFG parser, and the variations in stack trace formats across issue reports. Our replication package contains the details of the assessment.

The content marked with \citerespexp{MC-2} is the location of the change. \\

\noindent {\review{Point3:  Extend the final survey evaluation to a larger sample size.}}

Within the short span of one month of this revision, we were fortunate to increase the number of survey respondents from 11 to 31. We have added the following texts in the paper in Section \ref{sec:effectsurvey}.

A comparative study was conducted to assess the practical efficacy of CHIME, involving 31 participants. The majority (93\%) had 0-5 years of experience in the software industry, with 57\% being software developers and 33\% researchers.
Participants were presented with two random questions from each task in our benchmark dataset. The questions include a summarization of the failure of an issue, similarities between multiple issues, recurring themes in a component, pending issues, identification of error-prone components, unresolved or blocker issues, guidelines for labeling, and label suggestions. For these questions, responses from both CHIME and ChatGPT, along with links to associated bug reports, were provided for evaluation. To ensure a fair comparison, only questions with correct responses from both systems were selected. Participants were then asked to rate the correctness and perceived usefulness of the responses in addressing software bug-related queries. The survey questions are provided in our online appendix.

\noindent The content marked with \citerespexp{MC-3} is the location of the change. \\

\noindent {\review{Point4:  Provide clarity and additional details on: a) The ChatGPT setup b) The benchmark dataset creation process c) The issue report selection criteria d) The functioning of CFG e) The query transformation algorithm and process f) The response validator's process 5. Justify the assertion that 66.7\% accuracy is sufficient, and explain its practical applicability in real-world scenarios.}}

We have added the following texts in the paper in different locations to provide clarity and additional details on the above topics. The contents are marked with \citerespexpnopage{MC-4}. 

\textbf{The ChatGPT Setup.}
We used a temperature setting of 0. A temperature value above 0 produces slightly different answers to a prompt across multiple runs, which is unnecessary when we expect consistent answers from ChatGPT. We ran it multiple times on our benchmark dataset to ensure that the answers were indeed consistent across multiple runs.

\textbf{The Benchmark Dataset Creation Process.}
 In Table \ref{tab:bench-utility}, we showed a catalog of 23 questions that we validated with our survey participants and for which they wished for chatbot support. Each question is a template, which can be used to produce multiple similar questions. Based on the question templates in Table \ref{tab:bench-utility}, we produced a total of 412 questions from the issue reports of two popular OSS repos, OpenJ9 and ElasticSearch. OpenJ9 was chosen due to its alignment with our industrial partner. ElasticSearch \cite{es1,es2,es3} is frequently referenced in academic studies. We then produced an answer to each question by assessing the two OSS repos and by consulting among the authors. Four authors (the first two and last two) engaged in many hours of discussions that spanned over six months (both in-person and over formal presentations). The last two authors are also among the maintainers of OpenJ9. Given the benchmark was created via mutual discussion, we did not compute any standard agreement analysis metrics. 
 
\textbf{The Issue Report Selection Criteria.}
We created the benchmark by selecting 80 complex issues (40 from each repository). Following Deeksha et al. \cite{InfoTypesOSSDiscussion}, we define an issue as complex if it is excessively long and/or it has stack traces. We picked issues within the last year of our analysis because those are likely to be explored more by developers. We sorted issues by length and selected 40 issues with stack traces (per repo).

\textbf{The Functioning of CFG.}
We developed a CFG as shown in Listing \ref{lst:stack_trace_grammar} which supports parsing stack traces to the level of individual code elements. Stack traces can also contain auxiliary information like timestamps and memory addresses (e.g., crash dumps). We preprocessed these auxiliary information and applied our CFG to parse the code elements in a Java stack trace. Finally, our issue preprocessor stored the code blocks in the database by separating the code blocks from the textual contents. The issue preprocessor saves the following information by parsing an issue report: title, body, stack trace, and other metadata (creation date, status, etc).

\textbf{The Query Transformation Algorithm and Process.}
Each query goes through this component for error correction as follows. We prompt ChatGPT with instructions on how to transform a query based on the question type. For example, for a Yes/No query type, we instruct ChatGPT as follows ``Change `is/are/have there issues' to check if there are any issues with the provided condition''. For a summarization type question, the instruction is ``Summarize the contents from issue title, exceptions, body, and labels''. 
We then provide some example transformations (in a few-shot setting) to clarify the instruction, like the following.

\qabox{Query Preprocessor.}{\textbf{Original Query:} Are issue 18102 and 18669 similar?} { \textbf{Transformed Query:} Compare the exceptions, stack traces, and descriptions of issues 18102 and 18669 to determine similarity.}

Finally, GPT answers based on the transformed query.\\
\textbf{The Response Validator’s Process.}
The third component of CHIME is added to validate initial responses from RAG-based ChatGPT. We employed two strategies sequentially, CoVe \cite{dhuliawala2024chainofverification} and Metamorphic Testing (MT) \cite{Chen-MTSurvey-CSUR2018}.  Drawing inspiration from investigative interrogation techniques, CoVe's methodology is designed to test the consistency and authenticity of ChatGPT's responses through a series of challenge questions. CoVe's process can be unfolded into three distinct stages \begin{inparaenum} \item Upon receipt of a query, ChatGPT formulates an initial response based on its interpretation of the query within the context of available data. \item CoVe then autonomously generates a set of follow-up questions related to the initial response. CoVe dynamically determines the number of follow-up questions. These questions aim to clarify its preceding statements. \item The subsequent responses are analyzed for consistency with the initial response. Any observed contradictions signal the need for a review and adjustment of the initial response, leading to the refinement or generation of a new, more accurate answer. \end{inparaenum} 

However, CoVe can discard correct responses (if not found in responses to challenge questions) or promote incorrect responses (if responses are found both in base and challenge questions). We thus refine CoVe with MT as follows.

Using CoVe to verify ChatGPT's initial responses, we get an intermediate response which is then passed for consistency verification to MT. Central to MT is the concept of metamorphic relations (MRs), which involve applying transformations to input queries to anticipate changes in output. In CHIME, this approach is leveraged to introduce nuanced variations to the queries for testing the consistency of its responses under diverse conditions. A specific implementation of MRs in CHIME involves Sentence-Level Mutation, where equivalent questions are generated to test. This process includes \begin{inparaenum} \item using predefined MRs to subtly alter the phrasing or focus of the original queries.  In our implementation, MT generates three mutated questions each time in CHIME. For instance, the original query might be ``What causes error X in module Y?'', and its mutated equivalent could be ``Why does error X occur in module Y?''. \item The responses ChatGPT provides for both the original and mutated queries are compared to assess consistency with MR expectations. If an MR implies that adding specific details should refine the response, the evaluation checks for this level of refinement. After the refinement via MR, CHIME generates the final response for the users. \end{inparaenum} The user in CHIME does not see the mutated questions from CoVe or the mutated questions from MRs. Instead, the user only sees the final response from CHIME. However, CHIME can print the mutated questions to the user if needed.\\

\noindent {\review{Point5: Justify the assertion that 66.7\% accuracy is sufficient, and explain its practical applicability in real-world scenarios.}}

We added the following texts in the paper in Section \ref{sec:conclusion}  to address this comment. The content marked with \citerespexp{MC-5} is the location of the change. 

Our industrial partner is working on deploying CHIME as a Slack bot. The conceptualization of CHIME originated from an internal demo of a similar chatbot created by our partner one year ago. Their initial chatbot lacked the required accuracy, which we sought to address by developing CHIME. To further motivate the need for such a chatbot beyond our industrial partner, we conducted a survey of 47 software practitioners (see Section \ref{sec:chatbotneed}). The survey findings highlight the necessity of such chatbots in the real world. Feedback from 31 industry participants, presented in Section \ref{sec:effectsurvey} shows that CHIME is preferred for its ability to analyze, summarise, and label issues. Our industrial partner was involved in the design and evaluation of CHIME, which was crucial for advancing CHIME from the proof-of-concept stage to the current deployment stage within the company. Like any innovation, we expect to improve CHIME in an agile manner, i.e., based on user feedback once deployed.\\


\noindent {\review{Point6:  Include a background section to contextualize the research.}}

We defined hallucinations as irrelevant or incorrect responses at the first sentences in the abstract and Section \ref{sec:introdcution}. Next, to provide clearer context/background for this concept and relevance of this work in regards to other work, we have moved the related work section (previous Section VIII) to follow Section \ref{sec:related-work}. The content marked with \citerespexp{MC-6} is the location of the change. \\

\noindent {\review{Point7:  Enhance overall presentation quality: (1) Conduct a thorough edit to rectify grammatical errors (2) Improve clarity and readability throughout the paper.}

We have carefully rectified grammatical errors, typos, figure legend mismatches, keyword introductions (e.g., KQ), and other inconsistencies. Additionally, we sought to improve the clarity and readability of the paper.\\
%\noindent The content marked with \citerespexp{R-5} is the location of the change. \\


\noindent \textbf{Additional Comments by Reviewer-A (RA\#)}\\

\noindent {\review{RA1. The evaluation in Section VI.C is limited, with only a total of 10 questions from 5 tasks, which may not provide a comprehensive assessment of the approach's preferences over ChatGPT.}
}\\
\noindent While the number of questions may seem limited, we specifically selected questions that provide qualitative responses rather than simple yes/no or factual ones. This approach aimed at capturing nuanced aspects and performances of the two underlying systems (i.e, ChatGPT and CHIME). We thus ensured that there should be equal representation from each of the 5 tasks for the two systems. To further strengthen the evaluation, we also increased the number of survey respondents from 11 to 31. We understand that more survey questions might have offered additional insights. However, that would also have increased the survey response time, which could have discouraged the (busy) respondents from participating altogether.\\

\noindent {\review{RA2. As language models like ChatGPT continue to evolve rapidly, how do the authors envision adapting or extending CHIME to work with more advanced versions, such as GPT-4 or future iterations? What challenges might arise in this adaptation process?}}\\
\noindent We added the following texts in the paper in Section \ref{sec:chime}. The content marked with \citerespexp{RA-2} is the location of the change.

CHIME treats ChatGPT as an API, where the inputs (questions) and outputs (answers) are processed for inaccuracy detection and mitigation. We can use another LLM as an API in CHIME and apply all the techniques we developed. Doing so would simply require changing the API endpoints to point to the other LLM within the LangChain toolkit. CHIME will need to be updated significantly while using multi-modal LLMs, e.g., to process/validate modalities other than texts, etc.\\

\noindent \textbf{Additional Comments by Reviewer-B (RB\#)}\\

\noindent {\review {RB1. Tables are inconsistent. Some are in color with different fonts and then there are the tables, that are the traditional Latex tables that are black \& white with consistent fonts to the paper.}}\\
\noindent All the tables (except Table \ref{tab:bench-utility}) are black and white. We highlighted some rows in a table with gray color for ease of understanding of the results by the readers. Table \ref{tab:bench-utility} shows the perceived usefulness of each benchmark question template using three colors. We could change those colors into shades of black/gray if suggested by the reviewer.\\

\noindent {\review{RB2.  I would have preferred the research questions to be introduced earlier in the paper. Introducing them upfront would enhance the introduction and provide helpful context. Later, when they are revisited, a brief mention with just enough detail would suffice, eliminating the need to refer back to the initial introduction.}
}\\
\noindent We structured the introduction to outline the study in three distinct phases, where we provide a brief overview of each phase. By introducing the research questions later and within the context of each phase, we sought to maintain a coherent flow and provides more relevant context when they are revisited. We thus kept this flow in the revised manuscript.\\

\noindent {\review{RB3. How do you envision extending CHIME to handle other types of technical documents beyond bug reports?}}
\noindent We added the following texts in the paper in Section \ref{sec:conclusion}  to address this comment. The content marked with \citerespexp{RB-3} is the location of the change. 

To handle other documents, in CHIME we will improve the issue preprocessor module e.g., to separate code and textual contents, and to adapt the CFG to handle code snippets/traces/crash dumps in those documents or using a static partial program analyzer to handle code examples in API documentation. We expect that the other modules in CHIME can be used with minimal changes.\\

\noindent \textbf{We have addressed all comments from Reviewer-C when we addressed the metareview questions and comments.}\\

==> styles.tex <==
%\documentclass[sigconf,screen,anonymous]{acmart}
\usepackage[outercaption]{sidecap}    
\usepackage[figuresright]{rotating}
\usepackage{booktabs}
\usepackage{soul}
\usepackage{subfigure}
\usepackage{pgfplots}
\usepackage{pgfplotstable}
\usepackage[export]{adjustbox}
\pgfplotsset{width=5.5cm}
\usepackage[framemethod=TikZ]{mdframed} % noteboxes, boxes, etc.

%%
%% \BibTeX command to typeset BibTeX logo in the docs
\AtBeginDocument{%
  \providecommand\BibTeX{{%
    \normalfont B\kern-0.5em{\scshape i\kern-0.25em b}\kern-0.8em\TeX}}}

\hyphenation{op-tical net-works semi-conduc-tor}

\usepackage{balance}  % to better equalize the last page
\usepackage{graphics} % for EPS, load graphicx instead
%\usepackage[T1]{fontenc}
%\usepackage{txfonts}
%\usepackage{times}    % comment if you want LaTeX's default font
%\usepackage[pdftex]{hyperref}
% \usepackage{url}      % llt: nicely formatted URLs
\usepackage{color}
%\usepackage{textcomp}
\usepackage{booktabs}
\usepackage{ccicons}

%\usepackage{cite}
\usepackage{url}
\usepackage{fancybox}
\usepackage{multirow}
\usepackage{flushend}
\usepackage{booktabs}
\usepackage{tabularx}
\usepackage{comment}
\usepackage{array}
\usepackage[flushleft]{threeparttable}
\usepackage{mdframed}
\graphicspath{{}{images/}{dia/}}
\DeclareGraphicsExtensions{.pdf,.png,.svg}


\usepackage{listings}
\usepackage{courier}
\usepackage{hyperref}
\usepackage{xpatch}
\xdef\scr{}

\xpatchcmd{\refstepcounter}{%
  \stepcounter{#1}%
}{%
  \stepcounter{#1}%
  \xdef\scr{\number\value{#1}}%
}{\typeout{success}}{\typeout{failure}}


\newcounter{o}
\setcounter{o}{0}

\usepackage{tikz}
%colors
\definecolor{1c1}{RGB}{188,162,6}
\definecolor{1c2}{RGB}{137,129,80}
\definecolor{1c3}{RGB}{239,167,31}
\definecolor{1c4}{RGB}{88,194,241}
\definecolor{1c5}{RGB}{6,180,188}

\usepackage{listings}



% stiles used
\tikzset{mynode/.style={draw=white,solid,circle,fill=green,inner sep=1pt, thick,
text=black}}
%draw=black to get a black circle, fill=white so it actually has a
%background and text=black to not get that rendered in the specified color
\tikzset{arrow line/.style={dashed, line width= 2.5pt, color=#1}}
\usepackage{varwidth}
\def\bf{\textbf}
\def\eq {Equation~}
\def\eqm {Eq~}
\def\eqs {Equations~}
\def\fig {Figure~}
\def\figs {Figures~}
\def\tbl {Table~}
\def\tbls {Tables~}
\def\ie{\textit{i.e.,}}
\def\eg{\textit{e.g.,}}
\def\sec {Section~}
\def\lst {Listing~}
\def\secs {Sections~}
\def\alg {Algorithm~}
\def\algs {Algorithms~}
\def\app {Appendix~}
\def\it{\textit}
\def\tr{\textrm}
\def\tt{\mct}
\def\up{$\uparrow$}
\def\dn{$\downarrow$}
\newcommand{\ib}[1]{{\textbf {\textit { #1}}}}
\newcommand{\ts}[1]{{\textsc {{ #1}}}}
\newcommand{\mct}[1]{{\footnotesize {\texttt {#1}}}}
\newcommand{\qu}[1]{{\it{``#1''}}}
\newcommand{\api}[1]{{\sf{\texttt\small{#1}}}}
\newcommand{\callout}[1]{{\vspace{1mm}\noindent{\fbox{\parbox{0.97\columnwidth}{#1}}}\vspace{1mm}}}
\usepackage{paralist}

\let\labelindent\relax

\newcommand{\nd}{\vspace{1mm}\noindent}
%\usepackage[small,bf]{caption}
%\usepackage[toc,page]{appendix}
\usepackage{tikz}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=1pt] (char) {#1};}}

 \lstset{
         frame=lines,
         basicstyle=\small\ttfamily, % Standardschrift
         numbers=left,               % Ort der Zeilennummern
         numberstyle=\small,          % Stil der Zeilennummern
         %stepnumber=2,               % Abstand zwischen den Zeilennummern
         numbersep=5pt,              % Abstand der Nummern zum Text
         tabsize=2,                  % Groesse von Tabs
        % extendedchars=true,         %
         breaklines=true,            % Zeilen werden Umgebrochen
%         keywordstyle=\color{black},
 %   	 frame=single,
 %        keywordstyle=[1]\textbf,    % Stil der Keywords
 %        keywordstyle=[2]\textbf,    %
 %        keywordstyle=[3]\textbf,    %
 %        keywordstyle=[4]\textbf,   \sqrt{\sqrt{}} %
         stringstyle=\color{white}\ttfamily, % Farbe der String
         showspaces=false,           % Leerzeichen anzeigen ?
         showtabs=false,             % Tabs anzeigen ?
         xleftmargin=17pt,
         framexleftmargin=17pt,
         framexrightmargin=5pt,
         framexbottommargin=4pt,
         %backgroundcolor=\color{lightgray},
         showstringspaces=false,      % Leerzeichen in Strings anzeigen ?
     %    escapeinside={\%*}{*)}
 }

\lstdefinestyle{inlinecode}{basicstyle={\ttfamily\scriptsize\bfseries}}
\renewcommand*{\bibfont}{\normalfont\normalsize\rmfamily}
\newcommand\code{\lstinline[style=inlinecode]}
\newcommand{\urls}[1]{{\scriptsize\url{#1}}}
\usepackage{tcolorbox}
\newcommand{\emt}[1]{\emph{``#1''}}
\newcommand{\rev}[1]{\textcolor{blue}{#1}}

\newcommand{\gias}[1]{\textcolor{red}{{[Gias: #1]}}}
\usepackage{paralist}
\usepackage[outercaption]{sidecap}
\usepackage{caption}
\usepackage [autostyle, english = american]{csquotes}
\MakeOuterQuote{"}
\newcounter{scn}
\setcounter{scn}{1}
\usepackage[shortlabels]{enumitem}
\usepackage{tikz}
%\usepackage{styles/modified-pgf-pie}
%\usepackage{styles/pgf-pie}
\usetikzlibrary{trees,positioning,shapes,shadows,arrows}
\usepackage[edges]{forest}
\usepackage{pgf-pie}
\usepackage{paralist}
%\usepackage{hyperref}
\usepackage{soul}
\usepackage[utf8]{inputenc}
\usepackage[english]{babel}
\usepackage{float}
\usetikzlibrary{positioning}

\usetikzlibrary{positioning,shadows}
\usepackage{balance}
\newcommand{\dq}[1]{\href{https://stackoverflow.com/questions/#1/}{$Q_{#1}$}}
\newcommand{\da}[1]{\href{https://stackoverflow.com/answers/#1/}{$A_{#1}$}}

\newif\ifpienumberinlegend
\pgfkeys{/number in legend/.code=
    \expandafter\let\expandafter\ifpienumberinlegend
    \csname if#1\endcsname
    \ifpienumberinlegend
    \let\legendbeforenumber\beforenumber
    \let\legendafternumber\afternumber
    \def\beforenumber##1\afternumber{}%
    \fi,
    /number in legend/.default=true
}
%colors
\definecolor{1c1}{RGB}{188,162,6}
\definecolor{1c2}{RGB}{137,129,80}
\definecolor{1c3}{RGB}{239,167,31}
\definecolor{1c4}{RGB}{88,194,241}
\definecolor{1c5}{RGB}{6,180,188}

\usepackage{tcolorbox}
\tcbuselibrary{listings,skins}
% stiles used
\tikzset{mynode/.style={draw=white,solid,circle,fill=green,inner sep=1pt, thick,
text=black}}
%draw=black to get a black circle, fill=white so it actually has a
%background and text=black to not get that rendered in the specified color
\tikzset{arrow line/.style={dashed, line width= 2.5pt, color=#1}}

\usepackage{bchart}
\usepackage{xcolor}


    
% \newtcolorbox{noteBox}{textmarker,
%     %borderline west={0pt}{0pt}{black},
%     borderline={0pt}{0pt}{black},
%     colback=white!-10!white}        
%\newcommand{\note}[1]{\begin{noteBox} \textbf{Finding \arabic{o}:} #1 \end{noteBox}}

%\newcommand{\nd}{\vspace{1mm}\noindent}
\tikzstyle{chart}=
[legend label/.style={font={\small},anchor=west,align=left},
legend box/.style={rectangle, draw, minimum size=5pt},
axis/.style={black,thin,->},
axis label/.style={anchor=east,font={\tiny}}]

\tikzstyle{bar chart}=[
chart, bar width/.code={
    \pgfmathparse{##1/2}
    \global\let\bar@w\pgfmathresult},
bar/.style={thin, draw=black},
bar label/.style={font={\bf\small},anchor=north},
bar value/.style={font={\footnotesize}},
bar width=.75,]

\tikzstyle{pie chart}=
[chart,
slice/.style={line cap=round, line join=round, thin, draw=black},
pie title/.style={font={}},
slice type/.style 2 args={
    ##1/.style={fill=##2},
    values of ##1/.style={}}]

\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}

\newcommand{\tempsum}{0}% reserve global name

\newcommand{\pye}[3][]{% #1=scope options, #2=title, #3=list of percent/legend
    \begin{scope}[#1]
        \pgfmathsetmacro{\curA}{0}
        \pgfmathsetmacro{\r}{1}
        \def\c{(0,0)}
        \node[pie title] at (270:1.3) {#2};
        \def\tempsum{0}
        \foreach \v/\s in{#3}{
          \pgfmathparse{\v+\tempsum}
          \global\let\tempsum=\pgfmathresult}
        \foreach \v/\s in{#3}{
            \pgfmathsetmacro{\deltaA}{\v/\tempsum*360}
            \pgfmathsetmacro{\nextA}{\curA + \deltaA}
            \pgfmathsetmacro{\midA}{(\curA+\nextA)/2}
            \path[slice,\s] \c
            -- +(\curA:\r)
            arc (\curA:\nextA:\r)
            -- cycle;
            \pgfmathsetmacro{\d}{min(1.2,max((1.5-0.1*\v) , .5)}

%%%            

%\pgfmathprintnumberto{#3}{\fnum} 
%\ifthenelse{\lengthtest{#3 pt < 10pt}}
%{\path (O) -- ++ (\midangle:\radius)
%node[inner sep=0,align=left,anchor=west,rotate=\midangle](nums#3)    {~~\fnum};}
%{\path (O) -- ++(\midangle:\innerpos) 
%node {\scalefont{#3}\beforenumber\fnum\afternumber};}         

%%%            
            \begin{pgfonlayer}{foreground}
                \path \c -- node[pos=\d,pie values,values of \s]{$\v\%$} +  (\midA:\r);
            \end{pgfonlayer}
            \global\let\curA\nextA}
    \end{scope}}

\newcommand{\legend}[2][]{
    \begin{scope}[#1]
        \path
        \foreach \n/\s in {#2}
            {
                  ++(0,-10pt) node[\s,legend box] {} +(3pt,0) node[legend label] {\n}
            }
        ;
    \end{scope}}
	
\def\test#1{%
    \ifnum #1 > 0
      #1
    \fi
}
\newcommand{\sevenbars}[7]{
{{\color{red}\rule{#1pt}{4pt}} \test{#1}}
{{\color{green}\rule{#2pt}{4pt}} \test{#2}}
{{\color{violet}\rule{#3pt}{4pt}} \test{#3}}
{{\color{orange}\rule{#4pt}{4pt}} \test{#4}}
{{\color{blue}\rule{#5pt}{4pt}} \test{#5}}
{{\color{teal}\rule{#6pt}{4pt}} \test{#6}}
{{\color{magenta}\rule{#7pt}{4pt}} \test{#7}}
}
\newcommand{\onebar}[2]{
{{\color{#1}\rule{#2pt}{4pt}}}
}
\newcommand{\lstbg}[3][0pt]{{\fboxsep#1\colorbox{#2}{\strut #3}}}
\lstdefinelanguage{diff}{
  morecomment=[f][\lstbg{red!20}]-,
  morecomment=[f][\lstbg{green!20}]+,
  morecomment=[f][\textit]{@@},
  %morecomment=[f][\textit]{---},
  %morecomment=[f][\textit]{+++},
}
%\usepackage{arydshln}
%\newcommand{\gias}[1]{\textcolor{red}{{[Gias: #1]}}}

\newcommand{\definebox}[2]{%
  \newcounter{#1}
  \newenvironment{#1}[1][]{%
    \stepcounter{#1}%
    \mdfsetup{%
        frametitle={%
            \tikz[baseline=(current bounding box.east),outer sep=0pt]
            \node[anchor=east,rectangle,fill=white]
            {\strut \MakeUppercase#1~\csname the#1\endcsname\ifstrempty{##1}{}{:~##1}};}}%
    \mdfsetup{innertopmargin=0pt,linecolor=#2,%
        linewidth=0.5pt,topline=true,
        frametitleaboveskip=\dimexpr-\ht\strutbox\relax,}%
    \begin{mdframed}[]\relax%
    }{\end{mdframed}}%
}


\definebox{Recommendation}{black}

\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
            \node[shape=circle,draw,inner sep=2pt] (char) {#1};}}










